V-Learning -- A Simple, Efficient, Decentralized Algorithm for Multiagent RL

A major challenge of multiagent reinforcement learning (MARL) is the curse of multiagents, where the size of the joint action space scales exponentially with the number of agents. This remains to be a bottleneck for designing efficient MARL algorithms even in a basic scenario with finitely many states and actions. This paper resolves this challenge for the model of episodic Markov games. We design a new class of fully decentralized algorithms -- V-learning, which provably learns Nash equilibria (in the two-player zero-sum setting), correlated equilibria and coarse correlated equilibria (in the multiplayer general-sum setting) in a number of samples that only scales with $\max_{i\in[m]} A_i$, where $A_i$ is the number of actions for the $i^{\rm th}$ player. This is in sharp contrast to the size of the joint action space which is $\prod_{i=1}^m A_i$. V-learning (in its basic form) is a new class of single-agent RL algorithms that convert any adversarial bandit algorithm with suitable regret guarantees into a RL algorithm. Similar to the classical Q-learning algorithm, it performs incremental updates to the value functions. Different from Q-learning, it only maintains the estimates of V-values instead of Q-values. This key difference allows V-learning to achieve the claimed guarantees in the MARL setting by simply letting all agents run V-learning independently.

==> BI.tex <==
%!TEX root = main.tex

\section*{Broader Impact}

As this is a theoretical contribution, we do not envision that our direct results will have a tangible societal impact. Our broader line of inquiry could impact a line of thinking about how to design more sample-efficient algorithms for multi-agent reinforcement learning, which could be useful towards making artificial intelligence more resource and energy efficient.

% Our broader line of inquiry could impact a line of thinking in a way that provides additional means to provide confidence intervals relevant for planning and learning.  There is an increasing needs for applications to understand planning under uncertainty in the broader context of safety and reliability, and POMDPs provide one potential framework.

% There are numerous applications in which uncertainty is a central component in planning. This broader line of inquiry could impact this line of thinking in way that emphases how strategic exploration should be coupled with uncertainty not only in the model but in the hidden state estimation. Any applications clearly need to understand these in the context of safety and reliability due to mis-specified models.

% \chijin{Please modify this}

==> CCE.tex <==
\section{General games}

\begin{algorithm}[t]
  % \setstretch{1.2}
     \caption{\textsc{Optimistic V-learning General Game}}
     \label{algorithm:V-GG}
     \begin{algorithmic}[1]
        \STATE {\bfseries Initialize:} for any $(s, a, h)$,
        $V_{h}(s)\setto H$, $N_{h}(s)\setto 0$, $\pi_h(a|s) \setto 1/A$.
        \FOR{episode $k=1,\dots,K$}
        \STATE receive $s_1$.
        \FOR{step $h=1,\dots, H$}
        \STATE take action $a_h \sim \pi_h(\cdot |s_h)$, observe reward $r_h$ and next state $s_{h+1}$.
        \STATE $t=N_{h}(s_h)\setto N_{h}(s_h) + 1$.
        \STATE $\tilde{V}_h(s_h) \setto (1-\alpha_t)\tilde{V}_h(s_h)+ \alpha_t(r_h+V_{h+1}(s_{h+1})+\beta_t)$.
        \STATE $V_h(s_h) \setto \min\{H, \tilde{V}_h(s_h)\}.
        $
        \STATE $\pi_h(\cdot | s_h) \leftarrow \textsc{Adv\_Bandit\_Update}(a_h, r_h+V_{h+1}(s_{h+1}))$ on $(s_h, h)$-th adversarial bandit. 
        \ENDFOR
        \ENDFOR
     \end{algorithmic}
  \end{algorithm}

\begin{algorithm}[t]
    \caption{Certified Policy $\hat{\pi}^K$}
    \label{algorithm:V-policy}
    \begin{algorithmic}[1]
      \STATE sample $k \leftarrow \text{Uniform}([K])$.
       \FOR{step $h=1, \dots,H$}
       \STATE observe $s_{h}$, and set $t \setto N^{k}_h(s_{h})$.
       \STATE sample $n \in [t]$ with $\P(n=i)=\alpha^i_t$.
       \STATE $k \setto k^n_{h}(s_{h})$.
       \STATE take action $\{a_{h,i}\}_{i=1}^m \sim \pi^{k}_h(\cdot|s_h)$ (the product of all the players' policy).
       \ENDFOR
    \end{algorithmic}
  \end{algorithm}

  \tiancheng{Can similarly define $\hat{\pi}_h$, see appendix for detail.}



% We run Nash V-learning for each player separately and output the nested policy as in Algorithm ~\ref{algorithm:V-policy}. For each player we define the bonus as $\beta_{t,j}:=c\sqrt{H^3A_j\iota/t}$, for large absolute constant $c$ and $\iota = \log (S\sum_{j}A_jT/\delta)$.








==> Q.tex <==
%!TEX root = main.tex

\section{Optimistic Nash Q-learning}
\label{sec:exp-SAB}

In this section, we present our first algorithm \emph{Optimistic Nash Q-learning} and its corresponding theoretical guarantees.

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Optimistic Nash Q-learning}
   \label{algorithm:Nash_Q}
   \begin{algorithmic}[1]
      \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
      $\up{Q}_{h}(s,a, b)\setto H$, $\low{Q}_{h}(s,a, b)\setto 0$,
      $N_{h}(s,a, b)\setto 0$,\\\qquad\qquad~~$\pi_h(a, b|s) \leftarrow 1/(AB)$.
      % \STATE \qquad\qquad\qquad\qquad\qquad\qquad 
      \FOR{episode $k=1,\dots,K$}
      \STATE receive $s_1$.
      \FOR{step $h=1,\dots, H$}
      \STATE take action $(a_h, b_h) \sim  \pi_h(\cdot, \cdot| s_h)$.
      \STATE observe reward $r_h(s_h, a_h, b_h)$ and next state
      $s_{h+1}$.
      \STATE $t=N_{h}(s_h, a_h, b_h)\setto N_{h}(s_h, a_h, b_h) + 1$.
      \STATE $\up{Q}_h(s_h, a_h, b_h) \setto (1-\alpha_t)\up{Q}_h(s_h, a_h, b_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\up{V}_{h+1}(s_{h+1})+\beta_t)$ \label{line:Q_up_update}
      \STATE $\low{Q}_h(s_h, a_h, b_h) \setto (1-\alpha_t)\low{Q}_h(s_h, a_h, b_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})-\beta_t)$
      \label{line:Q_low_update}
      \STATE $\pi_h(\cdot, \cdot|s_h) \setto \textsc{CCE}(\up{Q}_h(s_h, \cdot, \cdot), \low{Q}_h(s_h, \cdot, \cdot))$
      \STATE $\up{V}_h(s_h) \leftarrow (\D_{\pi_h}\up{Q}_h)(s_h); \quad \low{V}_h(s_h) \leftarrow (\D_{\pi_h} \low{Q}_h)(s_h)$.
      \ENDFOR
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\paragraph{Algorithm part I: learning values}
Our algorithm \emph{Optimistic Nash Q-learning} (Algorithm \ref{algorithm:Nash_Q}) is an optimistic variant of Nash Q-learning \cite{hu2003nash}. For each step in each episode, it (a) takes actions according to the previously computed policy $\pi_h$, and observes the reward and next state, (b) performs incremental updates on Q-values, and (c) computes new greedy policies and updates $V$-values.
% the algorithm first acts according to the policy $\pi_h$ previously computed. 
% We note that $\pi_h$ is a possibly correlated joint distribution over both players actions. The execution of $\pi_h$ may require a cooperation of both players in the training phase, which can be achieved in a self-play algorithm. 
Part (a) is straightforward; we now focus on explaining part (b) and part (c).

In part (b), the incremental updates on Q-values (Line \ref{line:Q_up_update}, \ref{line:Q_low_update}) are almost the same as standard Q-learning \cite{watkins1989learning}, except here we maintain two separate Q-values---$\up{Q}_h$ and $\low{Q}_h$, as upper and lower confidence versions respectively. We add and subtract a bonus term $\beta_t$ in the corresponding updates, which depends on $t = N_{h}(s_h, a_h, b_h)$---the number of times $(s_h, a_h, b_h)$ has been visited at step $h$. We pick parameter $\alpha_t$ and $\beta_t$ as follows for 
some large constant $c$ , and log factors $\iota$:
\begin{equation}\label{eq:hyper_Nash_Q}
\textstyle \alpha_t= (H+1)/(H+t), \qquad \beta_t=c\sqrt{H^3\iota/t}
\end{equation}
% \begin{equation}\label{eq:hyper_Nash_Q}
% \alpha_t=\frac{H+1}{H+t}, \qquad \beta_t=c\sqrt{\frac{H^3\iota}{t}}
% \end{equation}
In part (c), our greedy policies are computed using
% Finally, for the step to compute greedy policies, we can no longer compute the minimax policies for the current $Q$-value, since we now have both upper confidence $\up{Q}_h$ and lower confidence $\low{Q}_h$. It turns out we can replace this step by a procedure of finding 
a \emph{Coarse Correlated Equilibrium} (CCE) subroutine, which is first introduced by \cite{xie2020learning} to solve Markov games using value iteration algorithms. For any pair of matrices $\up{Q}, \low{Q} \in [0, H]^{A\times B}$, $\textsc{CCE}(\up{Q}, \low{Q})$ returns a distribution $\pi \in \Delta_{\cA \times \cB}$ such that
% \begin{equation*}
% \E_{(a, b) \sim \pi} \up{Q}(s, a, b) \ge \max_{a^\star} \E_{(a, b) \sim \pi} \up{Q}(s, a^\star, b), \qquad
% \E_{(a, b) \sim \pi} \low{Q}(s, a, b) \le \min_{b^\star} \E_{(a, b) \sim \pi} \low{Q}(s, a, b^\star)
% \end{equation*}
\begin{align}
\E_{(a, b) \sim \pi} \up{Q}(a, b) \ge& \max_{a^\star} \E_{(a, b) \sim \pi} \up{Q}(a^\star, b) \label{eq:CCE}\\
\E_{(a, b) \sim \pi} \low{Q}(a, b) \le& \min_{b^\star} \E_{(a, b) \sim \pi} \low{Q}(a, b^\star) \nonumber
\end{align}
It can be shown that a CCE always exists, and it can be computed by linear programming in polynomial time (see Appendix \ref{app:CCE} for more details).
% We compute CCE since it always exists, and can be computed in polynomial time (see Appendix \ref{app:prop} for more details). In contrast, finding a Nash equilibrium of a general-sum game is PPAD-complete \cite{daskalakis2013complexity}.
% \chijin{Come back to this later}

Now we are ready to state an intermediate guarantee for optimistic Nash Q-learning. We assume the algorithm has played the game for $K$ episodes, and  we use $V^k, Q^k, N^k, \pi^k$ to denote values, visitation counts, and policies \emph{at the beginning} of the $k$-th episode in Algorithm \ref{algorithm:Nash_Q}.
% There are several unspecified parameters in Algorithm~\ref{algorithm:Nash_Q}. The step size is defined by $$. 

\begin{lemma}  \label{lem:regret_Nash_Q}
  For any $p\in (0, 1]$, choose hyperparameters $\alpha_t, \beta_t$ as in \eqref{eq:hyper_Nash_Q} for a large absolute constant $c$ and $\iota = \log (SABT/p)$. Then, with probability at least $1-p$, Algorithm~\ref{algorithm:Nash_Q} has following guarantees
  \begin{itemize}
  \item $\up{V}_{h}^{k}(s) \ge V^{\star}_{h}(s) \ge \low{V}_{h}^{k} (s)$ for all $(s, h, k) \in \cS \times [H]\times [K] $.
  \item $(1/K)\cdot\sum_{k=1}^K( \up{V}_{1}^{k}-\low{V}_{1}^{k} ) ( s_1 )  \le \cO\paren{\sqrt{H^5SAB\iota/K}}$.
  \end{itemize}
\end{lemma}
% \vspace{-5ex}
Lemma \ref{lem:regret_Nash_Q} makes two statements. First, it claims that the $\up{V}_{h}^{k}(s)$ and $\low{V}_{h}^{k} (s)$ computed in Algorithm~\ref{algorithm:Nash_Q} are indeed upper and lower bounds of the value of the Nash equilibrium. Second, Lemma \ref{lem:regret_Nash_Q} claims that the averages of the upper bounds and the lower bounds are also very close to the value of Nash equilibrium $V_1^\star(s_1)$, where the gap decrease as $1/\sqrt{K}$. This implies that in order to learn the value $V_1^\star(s_1)$ up to $\epsilon$-accuracy, we only need $\cO(H^5 SAB\iota/\epsilon^2)$ episodes.

However, Lemma \ref{lem:regret_Nash_Q} has a significant drawback: it only guarantees the learning of the \emph{value} of Nash equilibrium. It does not imply % any guarantees on the 
that the policies $(\mu^k, \nu^k)$ used in Algorithm \ref{algorithm:Nash_Q} are close to the Nash equilibrium, 
% as in Definition \ref{def:epsilon_Nash}, 
which requires the policies to have a near-optimal performance even against their best responses. This is a major difference between Markov games and standard MDPs, and is the reason why standard techniques from the MDP literature does not apply here. To resolve this problem, we propose a novel way to extract a certified policy from the optimistic Nash Q-learning algorithm.

\begin{algorithm}[t]
   \caption{Certified Policy $\hat{\mu}$ of Nash Q-learning}
   \label{algorithm:Q-policy}
   \begin{algorithmic}[1]
   \STATE sample $k \leftarrow \text{Uniform}([K])$.
      \FOR{step $h=1, \dots,H$}
      \STATE observe $s_{h}$, and take action $a_{h} \sim \mu^{k}_h(\cdot|s_h)$. 
      \STATE observe $b_{h}$, and set $t \setto N^{k}_h(s_{h},a_{h},b_{h})$.
      \STATE sample $m \in [t]$ with $\P(m=i)=\alpha^i_t$.
      \STATE $k \setto k^m_{h}(s_{h},a_{h},b_{h})$
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\paragraph{Algorithm part II: certified policies}
We describe our procedure of executing the certified policy $\hat{\mu}$ of the max-player is described in Algorithm \ref{algorithm:Q-policy}. Above, $\mu^k_h, \nu^k_h$ denote the marginal distributions of $\pi^k_h$ produced in Algorithm \ref{algorithm:Nash_Q} over action set $\cA, \cB$ respectively. We also introduce the following quantities that directly induced by $\alpha_t$:
\begin{equation} \label{eq:alpha_parameter}
\textstyle \alpha_{t}^{0}:=\prod_{j=1}^t{\left( 1-\alpha _j \right)}, \,\, \alpha _{t}^{i}:=\alpha _i\prod_{j=i+1}^t{\left( 1-\alpha _j \right)}
\end{equation}
whose properties are listed in the following Lemma~\ref{lem:step_size}. Especially, $\sum_{i=1}^t \alpha_t^i = 1$, so $\{\alpha_t^i\}_{i=1}^t$ defines a distribution over $[t]$.  We use $k^m_{h}(s,a,b)$ to denote the index of the episode where $(s,a,b)$ is observed in step $h$ for the $m$-th time. The certified policy $\hat{\nu}$ of the min-player is easily defined by symmetry. We note that $\hat{\mu}, \hat{\nu}$ are clearly general policies, but they are no longer Markov policies.

The intuitive reason why such policy $\hat{\mu}$ defined in Algorithm \ref{algorithm:Q-policy} is certified by Nash Q-learning algorithm, is because the update equation in line \ref{line:Q_up_update} of Algorithm \ref{algorithm:Nash_Q} and equation \eqref{eq:alpha_parameter} gives relation:
\begin{equation*}
   \textstyle \up{Q}_{h}^{k}(s,a,b)=\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+\up{V}_{h+1}^{k_h^i(s,a,b)}(s_{h+1}^{k_h^i(s,a,b)}) +\beta_i \right]}
\end{equation*}
This certifies the good performance against the best responses if the max-player plays a mixture of policies $\{\mu_{h+1}^{k_h^i(s,a,b)}\}_{i=1}^t$ at step $h+1$ 
% (since $\up{V}_{h+1}^{k_i}(s_{h+1}^{k_i})$ is computed by playing $\mu_{h+1}^{k_i}$ at step $h+1$) 
with mixing weights $\{\alpha_t^i\}_{i=1}^t$ (see Appendix \ref{app:Q_policy} for more details). 
A recursion of this argument leads to the certified policy $\hat{\mu}$---a nested mixture of policies.

We now present our main result for Nash Q-learning, using the certified policies $(\hat{\mu}, \hat{\nu})$.
% We can prove following sample complexity result for the certified policies $(\hat{\mu}, \hat{\nu})$. 
% which gives our main result in this section.
% We denote $V^k, Q^k, N^k, \pi^k$ for values and policies \emph{at the beginning} of the $k$-th episode.
\begin{theorem}[Sample Complexity of Nash Q-learning]
  \label{thm:sample_Nash_Q}
  For any $p\in (0,1]$, choose hyperparameters $\alpha_t, \beta_t$ as in \eqref{eq:hyper_Nash_Q} for large absolute constant $c$ and $\iota = \log (SABT/p)$.  Then, with probability at least $1-p$, if we run Nash Q-learning (Algorithm~\ref{algorithm:Nash_Q}) for $K$ episodes where
  \begin{equation*}
  \textstyle K \ge \Omega\left(H^5 SAB\iota/\epsilon^2\right),
  \end{equation*}
  the certified policies $(\hat{\mu}, \hat{\nu})$ (Algorithm \ref{algorithm:Q-policy}) will be $\epsilon$-approximate Nash, i.e. $V^{\dagger, \hat{\nu}}_1(s_1) - V^{\hat{\mu}, \dagger}_1(s_1) \le \epsilon$.
\end{theorem}
Theorem \ref{thm:sample_Nash_Q} asserts that if we run the optimistic Nash Q-learning algorithm for more than $\cO(H^5 SAB\iota/\epsilon^2)$ episodes, the certified policies $(\hat{\mu}, \hat{\nu})$ extracted using Algorithm \ref{algorithm:Q-policy} will be $\epsilon$-approximate Nash equilibrium (Definition \ref{def:epsilon_Nash}).

We make two remarks. First, the executions of the certified policies $\hat{\mu}, \hat{\nu}$ require the storage of $\{\mu^k_h\}$ and $\{\nu^k_h\}$ for all $k, h \in [H] \times [K]$. This makes the space complexity of our algorithm scales up linearly in the total number of episodes $K$. Second, Q-learning style algorithms (especially online updates) are crucial in our analysis for achieving sample complexity linear in $S$. They enjoy the property that every sample is only been used once, on the value function that is independent of this sample. 
% In line \ref{line:Q_up_update} of Algorithm \ref{algorithm:Nash_Q}, the new sample $s_{h+1}$ is independent of randomness in the upper bound $\up{V}_{h+1}$. 
% This is key in obtaining sample complexity linear in $S$. 
In contrast, value iteration type algorithms do not enjoy such an independence property, which is why the best existing sample complexity scales as $S^2$ \citep{bai2020provable}. \footnote{Despite \cite{azar2017minimax} provides techniques to improve the sample complexity from $S^2$ to $S$ for value iteration in MDP, the same techniques can not be applied to Markov games due to the unique challenge that, in Markov games, we aim at finding policies that are good against their best responses.}


% Finally, we remark that for computational complexity, since CCE can be computed in polynomial time, the overall runtime is clearly polynomial. For space complexity, the executions of the certified policies $\hat{\mu}, \hat{\nu}$ require the storage of $\{\mu^k_h\}$ and $\{\nu^k_h\}$ for all $k, h \in [H] \times [K]$. Adding the storage of $Q$-value in Algorithm \ref{algorithm:Nash_Q}, the leading order terms in space complexity are $\cO(HS(A+B)K + HSAB)$. We no longer enjoy the advantage of model-free algorithm in space complexity, which typically scales as $\cO(HSA)$ in MDP, independent of $K$. However, the most important benefit of Q-learning here is its nature of a online algorithm, where in line \ref{line:Q_up_update} of Algorithm \ref{algorithm:Nash_Q}, the new sample $s_{h+1}$ is independent of randomness in the upper bound $\up{V}_{h+1}$. This is key in obtaining sample complexity linear in $S$. In contrast, value iteration algorithm does not enjoy a similar independency property, which results in the best existing sample complexity scaling up with $S^2$ \citep{bai2020provable}. \footnote{Despite \cite{azar2017minimax} provides techniques to improve the sample complexity from $S^2$ to $S$ for value iteration in MDP, the same techniques can not be applied to Markov games due to the unique challenge that, in Markov games, we aim at finding policies that are good against their best responses.}

% \chijin{Talk about the certified upper bound or non-certified upper bound, and why we need to do this complicated policy here.}

% \chijin{Discuss why VI does not work over certified approach in the end.}

% \chijin{Talk about drawback on the space complexity}







==> V.tex <==
%!TEX root = main.tex
%!TEX root = main.tex


\section{Optimistic Nash V-learning}
\label{sec:exp-SA+B}

In this section, we present our new algorithm \emph{Optimistic Nash V-learning} and its corresponding theoretical guarantees. This algorithm improves over Nash Q-learning in sample complexity from $\tlO(SAB)$ to $\tlO(S(A+B))$, when only highlighting the dependency on $S, A, B$. 
% The complexity of the new algorithm matches the minimax lower bound up to $\poly(H)$ and log factors, for the first time.

% \begin{algorithm}[t]
% % \setstretch{1.2}
%    \caption{Optimistic Nash V-learning}
%    \label{algorithm:Nash_V}
%    \begin{algorithmic}[1]
%       \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
%       $\up{V}_{h}(s)\setto H$, $\low{V}_{h}(s)\setto 0$,
%       $\up{L}_h(s,a) \setto 0$, $\low{L}_h(s,b) \setto 0$,\\
%       \qquad\qquad~~$N_{h}(s)\setto 0$, $\mu_h(a|s) \setto 1/A$, $\nu_h(b|s) \setto 1/B$.
%       \FOR{episode $k=1,\dots,K$}
%       \STATE receive $s_1$.
%       \FOR{step $h=1,\dots, H$}
%       \STATE take action $a_h \sim \mu_h(\cdot |s_h)$, $b_h \sim \nu_h(\cdot| s_h)$.
%       \STATE observe reward $r_h(s_h, a_h, b_h)$ and next state
%       $s_{h+1}$.
%       \STATE $t=N_{h}(s_h)\setto N_{h}(s_h) + 1$.
%       \STATE $\up{V}_h(s_h) \setto (1-\alpha_t)\up{V}_h(s_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\up{V}_{h+1}(s_{h+1})+\up{\beta}_t)$.
%       \STATE $\low{V}_h(s_h) \setto (1-\alpha_t)\low{V}_h(s_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})-\low{\beta}_t)$
%       \FOR{all $a \in \cA$}
%       \STATE $\up{\ell}^t_h(s_h, a) \setto [H-r_h(s_h, a_h, b_h)-\up{V}_{h+1}(s_{h+1})] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_t]$.
%       % \STATE $\mu_h(a|s_h) \propto \exp[-(\eta_t/\alpha_t) \sum_{i=1}^t \alpha^i_t \cdot \up{\ell}^i_h(s_h, a)]$.
%       \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
%       \ENDFOR
%       % \STATE \textbf{for} all $a \in \cA$, let $\mu_h(a|s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_h( s_h, a)]$.
%       \STATE set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_h( s_h, \cdot)]$.
%       \FOR{all $b \in \cB$}
%       \STATE $\low{\ell}^t_h(s_h, b) \setto [r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})] \mathbb{I}\{b_h=b\}/[\nu_h(b_h|s_{h}) +\low{\eta}_t]$.
%       % \STATE $\nu_h(b|s_h) \propto \exp[-(\eta_t/\alpha_t) \sum_{i=1}^t \alpha^i_t \cdot \low{\ell}^i_h(s_h, b)]$.
%       \STATE $\low{L}_h( s_h, b)  \setto ( 1-\alpha _t )\low{L}_h( s_h,b ) +\alpha_t \low{\ell}_h(s_h, b)$.
%       % \STATE $\low{L}_h( s_h,b)  \setto \left( 1-\alpha _t \right)\low{L}_h\left( s_h,b_h \right) +\alpha_t \frac{r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})}{\nu _h\left( s_{h},b_h \right) +\gamma _t}$ 
%       \ENDFOR
%       % \STATE \textbf{for} all $b \in \cB$, let $\nu_h(b |s_h) \propto \exp[-(\low{\eta}_t/\alpha_t) \low{L}_h( s_h, b)]$.
%       \STATE set $\nu_h(\cdot |s_h) \propto \exp[-(\low{\eta}_t/\alpha_t) \low{L}_h( s_h, \cdot)]$.
%       \ENDFOR
%       \ENDFOR
%    \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
% % \setstretch{1.2}
%    \caption{Optimistic Nash V-learning (the max-player version)}
%    \label{algorithm:Nash_V}
%    \begin{algorithmic}[1]
%       \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
%       $\up{V}_{h}(s)\setto H$, $\up{L}_h(s,a) \setto 0$, $N_{h}(s)\setto 0$, $\mu_h(a|s) \setto 1/A$.
%       \FOR{episode $k=1,\dots,K$}
%       \STATE receive $s_1$.
%       \FOR{step $h=1,\dots, H$}
%       \STATE take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $b_h$ from opponent.
%       \STATE observe reward $r_h(s_h, a_h, b_h)$ and next state
%       $s_{h+1}$.
%       \STATE $t=N_{h}(s_h)\setto N_{h}(s_h) + 1$.
%       \STATE $\up{V}_h(s_h) \setto \min\{H,(1-\alpha_t)\up{V}_h(s_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\up{V}_{h+1}(s_{h+1})+\up{\beta}_t)\}$.
%       \FOR{all $a \in \cA$}
%       \STATE $\up{\ell}_h(s_h, a) \setto [H-r_h(s_h, a_h, b_h)-\up{V}_{h+1}(s_{h+1})] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_t]$.
%       \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
%       \ENDFOR
%       \STATE set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_h( s_h, \cdot)]$. \label{line:MWupdate}
%       \ENDFOR
%       \ENDFOR
%    \end{algorithmic}
% \end{algorithm}


\paragraph{Algorithm description}
Nash V-learning combines the idea of Follow-The-Regularized-Leader (FTRL) in the bandit literature with the Q-learning algorithm in reinforcement learning. This algorithm does not require extra information exchange between players other than standard game playing, thus can be ran separately by the two players. We describe the max-player version in Algorithm~\ref{algorithm:Nash_V}. See Algorithm \ref{algorithm:Nash_V_min} in Appendix \ref{sec:pf_V} for the min-player version, where $\low{V}_h$, $\low{L}_h$, $\nu_h$, $\low{\eta}_t$ and $\low{\beta}_t$ are defined symmetrically.

% the communication between both players, other than observing the actions played by the opponents \tiancheng{I find this sentense a little bit confusing. Does it mean we need to observe the actions?}. Algorithm \ref{algorithm:Nash_V} gives the version of the algorithm for the max-player. The min-player runs a symmetric version of the algorithm with corresponding $\low{V}_h$, $\low{L}_h$, $\nu_h$, $\low{\eta}_t$ and $\low{\beta}_t$. For completeness, we provide the min-player version of the algorithm in Algorithm \ref{algorithm:Nash_V_min} in Appendix \ref{sec:pf_V}.

% For each step in each episode of Algorithm \ref{algorithm:Nash_V}, the max-player first take actions according to $\mu_h$ computed in the algorithm. Then the max-player observe the tuple $(s_h, a_h, b_h, r_h, s_{h+1})$\tiancheng{I guess we don't need $b_h$ actually?}, and performs an incremental update on the upper confidence version of $V$-value, instead of $Q$-value as in Nash Q-learning algorithm, thus we name this algorithm Nash V-learning. The remaining steps in Algorithm \ref{algorithm:Nash_V} is used to update the policy $\mu_h$. The agent first compute $\up{\ell}_h(s_h, \cdot)$ the importance weighted estimator of the loss at the current step, we add $\up{\eta}_t$ in the denominator to provide high probability guarantees instead of standard expectation guarantees. The agent then computes the weighted cumulative loss $\up{L}_h( s_h, \cdot)$. Finally the policy $\mu_h$ is computed using FTRL principle:

For each step in each episode, the algorithm (a) first takes action according to $\mu_h$, observes the action of the opponent, the reward, and the next state, (b) performs an incremental update on $\up{V}$, and (c) updates policy $\mu_h$. The first two parts are very similar to Nash Q-learning. In the third part, the agent first computes $\up{\ell}_h(s_h, \cdot)$ as the importance weighted estimator of the current loss. 
% we add $\up{\eta}_t$ in the denominator to provide high probability guarantees instead of standard expectation guarantees. The agent 
She then computes the weighted cumulative loss $\up{L}_h( s_h, \cdot)$. Finally, the policy $\mu_h$ is updated using FTRL principle:
\begin{equation*}
\textstyle \mu_h(\cdot|s_h) \leftarrow \argmin_{\mu \in \Delta_{\cA}} ~ \up{\eta}_t \la  \up{L}_h( s_h, \cdot), \mu\ra + \alpha_t \text{KL}(\mu \| \mu_0)
\end{equation*}
Here $\mu_0$ is the uniform distribution over all actions $\cA$. Solving above minimization problem gives the update equation as in Line \ref{line:MWupdate} in Algorithm \ref{algorithm:Nash_V}. In multi-arm bandit, FTRL can defend against adversarial losses, with regret independent of the number of the opponent's actions. This property turns out to be crucial for Nash V-learning to achieve sharper sample complexity than Nash Q-learning (see the analog of Lemma \ref{lem:regret_Nash_Q} in Lemma \ref{lem:regret_Nash_V}).

% \begin{algorithm}[t]
%    \caption{Certified Policy $\hat{\mu}$ of Nash V-learning}
%    \label{algorithm:V-policy}
%    \begin{algorithmic}[1]
%    \STATE sample $k \leftarrow \text{Uniform}([K])$.
%       \FOR{step $h=1, \dots,H$}
%       \STATE observe $s_{h}$, and set $t \setto N^{k}_h(s_{h})$.
%       \STATE sample $m \in [t]$ with $\P(m=i)=\alpha^i_t$.
%       \STATE $k \setto k^m_{h}(s_{h})$.
%       \STATE take action $a_{h} \sim \mu^{k}_h(\cdot|s_h)$.
%       \ENDFOR
%    \end{algorithmic}
% \end{algorithm}

Similar to Nash Q-learning, we also propose a new algorithm (Algorithm \ref{algorithm:V-policy}) to extract a certified policy from the optimistic Nash V-learning algorithm. The certified policies are again non-Markovian. We choose all hyperparameters as follows, for some large constant $c$ , and log factors $\iota$.
 \begin{equation} \label{eq:hyper_Nash_V}
  \alpha_t=\frac{H+1}{H+t}, \quad\up{\eta}_t = \sqrt{\frac{\log A}{At}}, \quad\low{\eta}_t = \sqrt{\frac{\log B}{Bt}}, \quad\up{\beta}_t=c\sqrt{\frac{H^4A\iota}{t}}, \quad\low{\beta}_t=c\sqrt{\frac{H^4B\iota}{t}},
\end{equation}
We now present our main result on the sample complexity of Nash V-learning.
%  This allows us to state our final guarantees for Nash V-learning.

% We choose parameters $\alpha_t$, $\up{\eta}_t$, $\up{\beta}_t$ and their min-player versions $\low{\eta}_t$, $\low{\beta}_t$ to be dependent on $t=N_h(s_h)$---the number of times $s_h$ is visited at step $h$, in the following form, for 
% some large constant $c$ , and log factors $\iota$.
%  \begin{equation} \label{eq:hyper_Nash_V}
%   \alpha_t=\frac{H+1}{H+t}, \quad\up{\eta}_t = \sqrt{\frac{\log A}{At}}, \quad\low{\eta}_t = \sqrt{\frac{\log B}{Bt}}, \quad\up{\beta}_t=c\sqrt{\frac{H^4A\iota}{t}}, \quad\low{\beta}_t=c\sqrt{\frac{H^4B\iota}{t}},
%   \end{equation} 
% In bandit literature, FTRL is an algorithm that can cope with even adversarial losses. The regret bound for FTRL does not depends the number of actions of the opponent. This turns out to be key for Nash V-learning to achieve the following sharp guarantees. 
% that this advantage can be adapted to the setting of reinforcement learning, which gives following guarantees.


% Lemma \ref{lem:regret_Nash_V} again asserts that $\up{V}_{h}^{k}(s)$ and $\low{V}_{h}^{k} (s)$ are the high confidence upper bound and lower bound of the value of Nash equilibrium $V^{\star}_{h}(s)$. Moreover, the gap between the averages of the upper bounds and the lower bounds---$\sum_{k=1}^K \up{V}_{1}^{k} (s_1) /K$ and $\sum_{k=1}^K \low{V}_{1}^{k} (s_1) /K$ to the value of Nash equilibrium $V^{\star}_{1}(s_1)$ only scales as $1/\sqrt{K}$. 
% Comparing to Lemma \ref{lem:regret_Nash_Q}, the upper bound in the second guarantee has one additional $\sqrt{H}$ factor, but improves the $\sqrt{AB}$ dependency to $\sqrt{A+B}$. This is crucial for Nash V-learning to achieve the near-optimal sample complexity.

% Similar to Nash Q-learning, Lemma \ref{lem:regret_Nash_V} does not directly provide guarantees on any policies to be approximate Nash equilibrium. The certified policy $(\hat{\mu}, \hat{\nu})$ extracted from Nash V-learning algorithm is given in Algorithm \ref{algorithm:V-policy}, which uses the same notation convention as in Section \ref{sec:exp-SAB}. Again, $(\hat{\mu}, \hat{\nu})$ are general policies, but not Markov policies. Now we are ready to state our main result in this section.

\begin{theorem}[Sample Complexity of Nash V-learning]
  \label{thm:sample_Nash_V}
  For any $p\in (0,1]$, choose hyperparameters as in \eqref{eq:hyper_Nash_V} for large absolute constant $c$ and $\iota = \log (SABT/p)$.  Then, with probability at least $1-p$, if we run Nash V-learning (Algorithm~\ref{algorithm:Nash_V} and \ref{algorithm:Nash_V_min}) for $K$ episodes with 
  \begin{equation*}
  \textstyle K \ge \Omega\left(H^6 S(A+B)\iota/\epsilon^2\right),
  \end{equation*}
  its induced policies $(\hat{\mu}, \hat{\nu})$ (Algorithm \ref{algorithm:V-policy}) will be $\epsilon$-approximate Nash, i.e. $V^{\dagger, \hat{\nu}}_1(s_1) - V^{\hat{\mu}, \dagger}_1(s_1) \le \epsilon$.
\end{theorem}

Theorem \ref{thm:sample_Nash_Q} claims that if we run the optimistic Nash V-learning for more than $\cO(H^6 S(A+B)\iota/\epsilon^2)$ episodes, the certified policies $(\hat{\mu}, \hat{\nu})$ extracted from Algorithm \ref{algorithm:V-policy} will be $\epsilon$-approximate Nash (Definition \ref{def:epsilon_Nash}). Nash V-learning is the first algorithm of which the sample complexity matches the information theoretical lower bound $\Omega(H^3S(A+B)/\epsilon^2)$ up to $\poly(H)$ factors and logarithmic terms.



% \chijin{Explain the intuitive connection between V-learning and Q-learning, relation in MDP?}


==> general.tex <==


  

==> intro_backup.tex <==
%!TEX root = main.tex

\section{Introduction}
\label{sec:introduction}

MARL important

Curse of multiagent

Decentralized algorithm

Question

Our results/contributions

% This paper studies \emph{competitive reinforcement learning}
% (competitive RL), that is, reinforcement learning with two or more
% agents taking actions simultaneously, but each maximizing
% their own reward.
% Competitive RL is a major branch of the more general
% setting of multi-agent reinforcement learning (MARL), with the
% specification that the agents have conflicting rewards (so that they
% essentially compete with each other) yet can be trained in a
% centralized fashion (i.e. each agent has access to the other agents'
% policies)~ ~\cite{crandall2005learning}.

% There are substantial recent progresses in competitive RL, in
% particular in solving hard multi-player games such as
% GO~\citep{silver2017mastering},
% Starcraft~\citep{vinyals2019grandmaster}, and Dota
% 2~\citep{openaidota}.  A key highlight in their approaches is the
% successful use of \emph{self-play} for achieving super-human
% performance in absence of human knowledge or expert opponents. These
% self-play algorithms are able to learn a good policy for all players
% from scratch through repeatedly playing the current policies against
% each other and performing policy updates using these self-played game
% trajectories. The empirical success of self-play has challenged the
% conventional wisdom that expert opponents are necessary for achieving
% good performance, and calls for a better theoretical understanding.

% In practice, many applications involve multi-agent RL.


A wide range of modern artificial intelligence challenges can be cast as a multi-agent reinforcement learning (multi-agent RL) problem, in which more than one agent performs sequential decision making in an interactive environment. Multi-agent RL has achieved significant recent success on traditionally challenging tasks, for example in the game of GO \citep{silver2016mastering,silver2017mastering}, Poker \citep{brown2019superhuman}, real-time strategy games \citep{vinyals2019grandmaster, openaidota}, decentralized controls or multiagent robotics systems \citep{brambilla2013swarm}, autonomous driving \citep{shalev2016safe}, as well as complex social scenarios such as hide-and-seek~\citep{baker2020emergent}.
In many scenarios, the learning agents even outperform the best human experts .

Despite the great empirical success, a major bottleneck for many existing RL algorithms is that they require a tremendous number of samples. For example, the biggest AlphaGo Zero model is trained on tens of millions of games and took more than a month to train~\citep{silver2017mastering}. While requiring such amount of samples may be acceptable in simulatable environments such as GO, it is not so in other sample-expensive real world settings such as robotics and autonomous driving. It is thus important for us to understand the \emph{sample complexity} in RL---how can we design algorithms that find a near optimal policy with a small number of samples, and what is the fundamental limit, i.e. the minimum number of samples required for any algorithm to find a good policy.

Theoretical understandings on the sample complexity for multi-agent RL are rather limited, especially when compared with single-agent settings. The standard model for a single-agent setting is an episodic Markov Decision Process (MDP) with $S$ states, and $A$ actions, and $H$ steps per episode. The best known algorithm can find an $\epsilon$ near-optimal policy in $\tilde{\Theta}({\rm poly}(H)SA/\epsilon^2)$ episodes, which matches the lower bound up to a single $H$ factor~\citep{azar2017minimax,dann2019policy}. In contrast, in multi-agent settings, the optimal sample complexity remains open even in the basic setting of two-player tabular Markov games \cite{shapley1953stochastic}, where the agents are required to find the solutions of the games---the Nash equilibria.
The best known algorithm, {\tt VI-ULCB}, finds an $\epsilon$-approximate Nash equilibrium in $\tlO({\rm poly}(H)S^2AB/\epsilon^2)$ episodes~\citep{bai2020provable}, where $B$ is the number of actions for the other player. The information theoretical lower bound is $\Omega({\rm poly}(H)S(A+B)/\epsilon^2)$. Specifically, the number of episodes required for the algorithm scales quadratically in both $S$ and $(A,B)$, and exhibits a gap from the linear dependency in the lower bound. 
This motivates the following question:
\begin{center}
  {\bf Can we design algorithms with near-optimal sample complexity for learning Markov games?}
\end{center}
In this paper, we present the first line of near-optimal algorithms for two-player Markov games that match the aforementioned lower bound up to a $\poly(H)$ factor. This closes the open problem for achieving the optimal sample complexity in all $(S,A,B)$ dependency. Our algorithm learns by playing against itself without requiring any direct supervision, and is thus a \emph{self-play} algorithm.


\subsection{Our contributions}
\begin{itemize}[leftmargin=*]
\item We propose an optimistic variant of \emph{Nash Q-learning} \cite{hu2003nash}, and prove that it achieves sample complexity $\tlO(H^5SAB/\epsilon^2)$ for finding an $\epsilon$-approximate Nash equilibrium in two-player Markov games (Section~\ref{sec:exp-SAB}). 
Our algorithm builds optimistic upper and lower estimates of $Q$-values, and computes the \emph{Coarse Correlated Equilibrium} (CCE) over this pair of $Q$ estimates as its execution policies for both players.

\item We design a new algorithm---\emph{Nash V-learning}---for finding approximate Nash equilibria, and show that it achieves sample complexity $\tlO(H^6S(A+B)/\epsilon^2)$ (Section~\ref{sec:exp-SA+B}). This improves upon Nash Q-learning in case $\min\set{A,B}>H$. It is also the first result that matches the minimax lower bound up to only a $\poly(H)$ factor. This algorithm builds optimistic upper and lower estimates of $V$-values, and features a novel combination of Follow-the-Regularized-Leader (FTRL) and standard Q-learning algorithm to determine its execution policies.

\item Apart from finding Nash equilibria, we prove that learning the best responses of fixed opponents in Markov games is as hard as learning parity with noise---a notoriously difficult problem that is believed to be computationally hard (Section~\ref{sec:lower}). As a corollary, this hardness result directly implies that achieving sublinear regret against \emph{adversarial opponents} in Markov games is also computationally hard, a result that first appeared in~\citep{radanovic2019learning}. This in turn rules out the possibility of designing efficient algorithms for finding Nash equilibria by running no-regret algorithms for each player separately.
\end{itemize}
In addition to above contributions, this paper also features a novel approach of extracting \emph{certified policies}---from the estimates produced by reinforcement learning algorithms such as Nash Q-learning and Nash V-learning---that are \emph{certified} to have similar performance as Nash equilibrium policies, even when facing against their best response (see Section \ref{sec:exp-SAB} for more details). We believe this technique could be of broader interest to the community.


==> lower.tex <==
%!TEX root = main.tex

\section{Hardness for Learning the Best Response}
\label{sec:lower}

In this section, we present a computational hardness result for computing the best response against an opponent with a fixed unknown policy. We further show that this implies the computational hardness result for achieving sublinear regret in Markov games when playing against adversarial opponents, which rules out a popular approach to design algorithms for finding Nash equilibria.

We first remark that if the opponent is restricted to only play Markov policies, then learning the best response is as easy as learning a optimal policy in the standard single-agent Markov decision process, where efficient algorithms are known to exist. Nevertheless, when the opponent can as well play any policy which may be non-Markovian, we show that finding the best response against those policies is computationally challenging.

% \chijin{We note that learning the best response for opponent who only plays Markov policies is easy, which can be reduced to the standard MDP. However, the opponent can for sure also plays non-Markovian policies, which makes it much more challenging to find the best response.}

We say an algorithm is a \emph{polynomial time algorithm for learning the best response} if for any policy of the opponent $\nu$, and for any $\epsilon > 0$, the algorithm finds the $\epsilon$-approximate best response of policy $\nu$ (Definition \ref{def:epsilon_best_response}) with probability at least $1/2$, in time polynomial in $S, H, A, B, \epsilon^{-1}$.

We can show the following hardness result for finding the best response in polynomial time.

\begin{theorem}[Hardness for learning the best response]
  \label{theorem:lower-bound-best-response}
There exists a Markov game with deterministic transitions and rewards defined for any horizon $H\ge 1$ with $S=2$, $A=2$, and $B=2$, such that if there exists a polynomial time algorithm for learning the best response for this Markov game, then there exists a polynomial time algorithm for learning parity with noise (see problem description in Appendix \ref{appendix:proof-lower}).
\end{theorem}

We remark that learning parity with noise is a notoriously difficult problem that has been used to design efficient cryptographic schemes.
It is conjectured by the community to be hard.
\begin{conjecture}[\cite{kearns1998efficient}]\label{conj:hardness}
There is no polynomial time algorithm for learning party with noise.
\end{conjecture}

Theorem \ref{theorem:lower-bound-best-response} with Conjecture \ref{conj:hardness} demonstrates the fundamental difficulty---if not strict impossibility---of designing a polynomial time for learning the best responses in Markov games. The intuitive reason for such computational hardness is that, while the underlying system has Markov transitions, the opponent can play policies that encode long-term correlations with non-Markovian nature, such as parity with noise, which makes it very challenging to find the best response. It is known that learning many other sequential models with long-term correlations (such as hidden Markov models or partially observable MDPs) is as hard as learning parity with noise \cite{mossel2005learning}.



\subsection{Hardness for Playing Against Adversarial Opponent}
% \chijin{1. Define no regret algorithm, 2. State conditional lower bound, 3. Clarify why this rule out a class of algorithms for learning Nash equilibrium.}

% In this section, we investigate a natural idea for solving two-player Markov games via combining two ``no-regret'' algorithms, and show that such an approach may be infeasible due to a computational lower bound for achieving no regret against adversarial opponents.

Theorem \ref{theorem:lower-bound-best-response} directly implies the difficulty for achieving sublinear regret in Markov games when playing against adversarial opponents in Markov games. Our construction of hard instances in the proof of Theorem \ref{theorem:lower-bound-best-response} further allows the adversarial opponent to only play Markov policies in each episode.
% , while keeping the problems remain computational challenging. 
Since playing against adversarial opponent is a different problem with independent interest, we present the full result here.

% In this section, we present a computational hardness result for achieving sublinear regret in Markov games when playing against adversarial opponents, and discuss its implications. 
% This result rules out the possibility of solving Markov games efficiently through running no-regret algorithms for each player separately.
 % We also discuss its implication on the design of 

% By ``one-sided'', we mean an algorithm that only controls one player but are guaranteed to achieve satisfactory performance (e.g. low regret) against an \emph{arbitrary} (potentially adversarial) opponent.

% \paragraph{Reduction to one-sided algorithms}
% We first show how a Markov game can be reduced to one-sided algorithms. Suppose there exists an algorithm that only controls the max-player, but is able to output policies $\mu^k$ that achieves the \emph{one-sided regret bound}
% \paragraph{No-regret algorithms against adversarial opponents}
Without loss of generality, we still consider the setting where the algorithm can only control the max-player, while the min-player is an adversarial opponent. In the beginning of every episode $k$, both players pick their own policies $\mu^k$ and $\nu^k$, and execute them throughout the episode. The adversarial opponent can possibly pick her policy $\nu^k$ \emph{adaptive} to all the observations in the earlier episodes. 

We say an algorithm for the learner is a \emph{polynomial time no-regret algorithm} if there exists a $\delta >0$ such that for \emph{any} adversarial opponent, and any fixed $K > 0$, the algorithm outputs policies $\{\mu^k\}_{k=1}^K$ which satisfies the following, with probability at least $1/2$, in time polynomial in $S, H, A, B, K$.
% For any algorithm that controls the max-player, we say it is a \emph{no-regret algorithm against adversarial opponents}, if in each episode $k$, it outputs policies $\mu^k$ that achieves the one-sided regret bound for \emph{any} opponent policy $\nu^k$ and some $\delta>0$:
\begin{equation}
  \label{equation:one-sided-regret}
  \Reg(K) = \sup_\mu \sum_{k=1}^K V^{\mu, \nu^k}_{1}
  (s_1) -  \sum_{k=1}^K V^{\mu^k, \nu^k}_{1} (s_1) \le {\rm poly}(S, H, A, B)K^{1-\delta}
\end{equation}

% for \emph{any} opponent policy $\nu^k$ and some $\delta\ge 0$. % In other words, a no-regret algorithm is one that is guaranteed to achieve sublinear regret in $K$ against the best possible policy in hindsight, regardless of how the opponent plays.

% We can show the following hardness results for designing polynomial time no-regret algorithms.
Theorem~\ref{theorem:lower-bound-best-response} directly implies the following hardness result for achieving no-regret against adversarial opponents, a result that first appeared in~\citep{radanovic2019learning}.
\begin{corollary}[Hardness for playing against adversarial opponent]
  \label{cor:lower-bound-coupled}
There exists a Markov game with deterministic transitions and rewards defined for any horizon $H\ge 1$ with $S=2$, $A=2$, and $B=2$, such that if there exists a polynomial time no-regret algorithm for this Markov game, then there exists a polynomial time algorithm for learning parity with noise (see problem description in Appendix \ref{appendix:proof-lower}).
The claim remains to hold even if we restrict the adversarial opponents in the Markov game to be non-adaptive, and to only play Markov policies in each episode.
\end{corollary}

Similar to Theorem \ref{theorem:lower-bound-best-response}, Corollary \ref{cor:lower-bound-coupled} combined with Conjecture \ref{conj:hardness} demonstrates the fundamental difficulty of designing a polynomial time no-regret algorithm against adversarial opponents for Markov games.
% A similar construction also appears in \cite{radanovic2019learning}.

% Theorem \ref{theorem:lower-bound-best-response}, combined with Conjecture \ref{conj:hardness}, demonstrates the fundamental difficulty---if not strict impossibility---of designing a polynomial time no-regret algorithm against adversarial opponents for Markov games. The intuitive reason for such computational hardness is that, while the underlying system has Markov transitions, the adversarial opponent can play policies that encode long-term correlations with non-Markovian nature, which makes it challenging to find the ``best response''. It is known that learning many other sequential models with long-term correlations (such as hidden Markov models or partially observable MDPs) is as hard as learning parity with noise \cite{mossel2005learning}.


\paragraph{Implications on algorithm design for finding Nash Equilibria}
% Perhaps surprisingly, Theorem~\ref{theorem:lower-bound-coupled} rules out the possibility of designing efficient algorithms for finding Nash equilibrium through combining two no-regret algorithms. Indeed, it is not hard to see that putting together two such algorithms (for both the max- and min-player) can yield a regret bound for finding Nash. However, Theorem~\ref{theorem:lower-bound-coupled} shows that achieving such no-regret is itself hard without additional knowledge about the opponent.
Corollary~\ref{cor:lower-bound-coupled} also rules out a natural approach for designing efficient algorithms for finding approximate Nash equilibrium through combining two no-regret algorithms. In fact, it is not hard to see that if the min-player also runs a non-regret algorithm, and obtain a regret bound symmetric to \eqref{equation:one-sided-regret}, then summing the two regret bounds shows the mixture policies $(\hat{\mu}, \hat{\nu})$---which assigns uniform mixing weights to policies $\{\mu^k\}_{k=1}^K$ and $\{\nu^k\}_{k=1}^K$ respectively---is an approximate Nash equilibrium. Corollary~\ref{cor:lower-bound-coupled} with Conjecture \ref{conj:hardness} claims that any algorithm designed using this approach is not a polynomial time algorithm.


% that putting together two such algorithms (for both the max- and min-player) can yield a regret bound for finding Nash. However, Theorem~\ref{theorem:lower-bound-coupled} shows that achieving such no-regret is itself hard without additional knowledge about the opponent.



% the following well-known conjecture on the hardness of learning parity with noise, which was heavily used to design efficient cryptographic.

% \paragraph{Computational lower bound for no-regret algorithms}
% % Perhaps surprisingly, we show in this section when the opponent policies $\nu^k$ are \emph{arbitrary} and potentially adversarial,
% We now show that achieving no regret in the sense of~\eqref{equation:one-sided-regret} can exhibit certain computational hardness, thereby demonstrating some fundamental difficulty---if not strict impossibility---for learning in Markov games against adversarial opponents.

% \begin{theorem}[Computational lower bound for no-regret algorithms]
%   \label{theorem:lower-bound-coupled}
%   There exists a Markov game with deterministic transitions and rewards defined for any horizon $H\ge 1$ with $S=2$, $A=2$, and $B=2$ such that the following holds: suppose there exist a deterministic algorithm that runs in ${\rm poly}(K,H)$ time and outputs policies $\mu^k$ such that
%   \begin{align*}
%     \sup_{\nu^k} \brac{ \sup_{\mu} \sum_{k=1}^K V_1^{\mu, \nu^k}(s_1) - \sum_{k=1}^K V_1^{\mu^k, \nu^k}(s_1) } \le {\rm poly}(H)K^{1-\delta}
%   \end{align*}
%   for some $\delta>0$, then there exist a polynomial time algorithm that achieves regret $\cO({\rm poly}(n)T^{1-\delta})$ in the online agnostic parity learning problem, where $n$ is the dimension of the input and $T$ is the number of rounds.
% \end{theorem}


% \begin{theorem}[Computational lower bound for no-regret algorithms (old)]
%   \label{theorem:lower-bound-coupled}
%   There exists a Markov game defined for any horizon $H\ge 1$ with $|\cS_h|\le 2$, $|\cA_h|\le 2$, and $|\cB_h|\le 2$ such that the following holds: suppose there exist an algorithm that runs in ${\rm poly}(K,H)$ time and outputs policies $\mu^k$ such that
%   \begin{align*}
%     \sup_{\nu^k} \E_{\mu^k}\brac{ \sup_{\mu} \sum_{k=1}^K V_1^{\mu, \nu^k}(s_1) - \sum_{k=1}^K V_1^{\mu^k, \nu^k}(s_1) } \le {\rm poly}(H)K^{1-\delta}
%   \end{align*}
%   for some $\delta>0$, then there exist a polynomial time algorithm for the agnostic parity learning problem that achieves regret $\cO({\rm poly}(n)T^{1-\delta})$ in the online agnostic parity learning problem, where $n$ is the dimension of the input and $T$ is the number of rounds.
% \end{theorem}
% \yubai{Comment on difference from Lemma 5: one-step vs. H steps, if Lemma 5 is shown in the main text.}
% \yubai{Briefly mention what parity learning is (in words or inline eqs.)}
% Conditioned on that achieving sublinear regret in the online agnostic parity learning problem is computationally hard (which it is believed to be~\citep{kalai2008agnostic}), Theorem~\ref{theorem:lower-bound-coupled} implies that achieving no-regret against adversarial opponents is also computationally hard.
% Our proof of Theorem~\ref{theorem:lower-bound-coupled} builds on a construction of single-player MDPs by~\citet{yadkori2013online} that simulate the online agnostic parity learning problem, and constructing a Markov game that (to the max player) simulates such a family of MDPs through a rich enough action space for the min-player. The full proof can be found in Appendix~\ref{appendix:proof-lower-bound-coupled}. % \yubai{polish descriptions.}


% Indeed, if we can design a no-regret algorithm for the max-player that achieves~\eqref{equation:one-sided-regret}, then by symmetry we can also design a no-regret algorithm for the min-player that achieves a same bound for ${\rm Regret}_{\min}(K)$. Summing these two bounds lead to a sublinear regret bound for finding Nash, which leads to a sample complexity guarantee as well.
% \begin{equation}
%     \label{equation:one-sided-regret-'}
%   \Reg_{\min}(K) = \sum_{k=1}^K V^{\mu^k, \nu^k}_{1} (s_1) - \inf_\nu \sum_{k=1}^K V^{\mu^k, \nu}_{1}(s_1) \le {\rm poly}(S, H, B, A)K^{1-\delta}.
% \end{equation}
% Letting the two algorithms play against each other and summing up~\eqref{equation:one-sided-regret} and~\eqref{equation:one-sided-regret-'}, we obtain the regret bound
% \begin{equation}
%   \label{equation:two-sided-regret}
%   \sup_\mu \sum_{k=1}^K V^{\mu, \nu^k}_{1}(s_1) - \inf_\nu \sum_{k=1}^K V^{\mu^k, \nu}_{1}(s_1) \le {\rm poly}(S, H, A, B)K^{1-\delta},
% \end{equation}
% which further implies that the policies $(\hat{\mu}, \hat{\nu}) = (\frac{1}{K}\sum_{k=1}^K \mu^k, \frac{1}{K}\sum_{k=1}^K \nu^k)$ are near Nash by the online-to-batch conversion~\citep{bai2020provable}.

% However, Theorem~\ref{theorem:lower-bound-coupled} shows that achieving the no-regret guarantees~\eqref{equation:one-sided-regret} and~\eqref{equation:one-sided-regret-'} against adversarial opponents is computationally challenging. 
% This implies that it is not possible to solve Markov games efficiently through putting two no-regret algorithms together in a black-box way, as the no-regret guarantee itself is computationally hard to achieve without additional knowledge about the opponent.




% \paragraph{Importance of self-play}
% Intriguingly, we note that Theorem~\ref{theorem:lower-bound-coupled} may have revealed the necessity of \emph{self-play} for designing efficient algorithms for Markov games---as achieving low one-sided regret against adversarial opponents is hard, it is perhaps necessary that the two players are not adversarial and have knowledge about each other's policies, which are exactly self-play algorithms.

% The astute reader may have noticed that our V-learning algorithm \yubai{ref} is also ``one-sided'' and may wonder whether our lower bound in Theorem~\ref{theorem:lower-bound-coupled} is contradictory to our main result. Indeed, in V-learning, each player builds its upper/lower estimates on its own which seemingly does not utilize knowledge about the opponent. However, the key difference is that such an agnosticity about the opponent is only \emph{one-step}: ~\yubai{to be continued.}


% \yubai{deprecated stuff blow.}

% Given this reduction, it is natural to ask the following
% \begin{quote}
%  {\bf Question}: \emph{Can we design an one-sided algorithm that achieves low regret~\eqref{equation:one-sided-regret} against any opponent, which (when playing two of them against each other) can achieve the regret bound~\eqref{equation:two-sided-regret}?}
% \end{quote}


% solving Markov games through these one-sided algorithms~\emph{without knowledge of the opponent}.
  
% Our lower bounds is stated for algorithms for the max-player in Markov games. More specifically, we consider the following two models for the max-player:
% \begin{enumerate}
% \item {\bf Uncoupled players}: After playing an action $a_h$, the max-player can see the reward $r_h$ and next state $s_{h+1}$, but not the min-player's action $b_h$. 
% \item {\bf Coupled players}: The max-player can see $(b_h, r_h, s_{h+1})$ after playing $a_h$.
% \end{enumerate}
% Clearly, the coupled setting reveals more observations to the max-player, and is thus easier than the uncoupled setting. We will show that one-sided regret bound~\eqref{equation:one-sided-regret} is statistically impossible to achieve in the uncoupled setting (Section~\ref{section:statistical-hardness}, and is computationally hard in the coupled setting (Section~\ref{section:computational-hardness}).



% \yubai{However, in this section we show such one-sided regrets could suffer from both statistical and computational hardness without structural assumptions on the MDPs and the opponents.}

% \yubai{Because adversarial MDPs involve changing opponents, we prove the lower bound in terms of the regret; there's no ``PAC'' guarantee in presence of adversarial opponents.}

% Now let us consider the case when we can only control one player. Define the one-side regret of the max-player by

% \begin{equation*}
%   \Reg(K) = \sup_\mu \sum_{k=1}^K V^{\mu, \nu^k}_{1}
%   (s_1) -  \sum_{k=1}^K V^{\mu^k, \nu^k}_{1} (s_1).
%   % \enspace
% \end{equation*}

% \yubai{this is the weak regret. however, strong regret for adversarial MDPs is meaningless.}

% \subsection{Statistical hardness for uncoupled players}

% \yubai{Remove this part.}

% We first consider the uncoupled setting where the max-player does not observe the min-player's actions. In this case, we show that the one-sided regret for the max-player has to be at least either linear in $K$ or exponential in $H$.
% \label{section:statistical-hardness}
% \begin{theorem}[Statistical hardness for uncoupled players]
%   \label{theorem:lower-bound-uncoupled}
%   For any $H\ge 2$ and $K\ge 1$, there exist a Markov game with horizon $H$, $|\cS_h|\le 2$, $|\cA_h|\le 2$, $|\cB_h|\le 4$ such that the following holds: any algorithm (in the uncoupled setting) will suffer from the following worst-case one-sided regret bound:
%   % that deploys policies $\mu^k$ in episode $k$ based on the seen states, rewards, but not the actions taken by the min player,
%   \begin{equation*}
%     \sup_{\nu^k} \E_{\mu^k} \brac{ \sup_{\mu} \sum_{k=1}^K V_1^{\mu, \nu^k}(s_1) - \sum_{k=1}^K V_1^{\mu^k, \nu^k}(s_1) } \ge \Omega\paren{\min\set{\sqrt{2^HK}, K}}.
%   \end{equation*}
%   In particular, any algorithm has to suffer from linear regret unless $K\ge \Omega(2^H)$.
% \end{theorem}
% Our proof builds on (1) constructing a ``combination lock'' type of hard MDPs for a single player and showing that an adversarial sequence of MDPs in this family is as hard as a bandit problem with $2^H$ arms, and (2) simulating such a family of MDPs via a suitable Markov game that has a ``rich enough'' action space for the min-player.
% The proof can be found in Appendix~\ref{appendix:proof-lower-bound-uncoupled}.
% % \yubai{Polish statement of result, and discuss.}

% \subsection{Computational hardness for coupled players}
% \label{section:computational-hardness}

% Now we consider the coupled setting, which is easier to the max-player as she gets to observe the min-player's actions. In this case, we show that achieving sublinear one-sided regret is still computationally challenging.

% The information revealed by the min-player's action makes the decision of the max-player easier. However, even in this case the problem is hard in a computational sense.

==> monotone_backup.tex <==
%!TEX root = main.tex

\section{Monotonic V-Learning}
\label{sec:monotone}






In the previous sections, we present the V-learning algorithm that outputs a nested mixture of Markov polices. However, storing such a nested policy in general leads to space complexity $\Omega(KH)$ which can be much larger than the space complexity of storing a Markov policy---$\cO(SAH)$. To avoid this space deficiency, we introduce a simple technique called \emph{monotone update} in this section. 
Below we show monotone update can be effortlessly combined with V-learning in the two-player zero-sum setting to obtain Markov output policy that enjoys the same sample-efficiency guarantee. Since MDPs is a special subclass of two-player zero-sum MGs, all the results in this section readily apply to MDPs by simply setting the action set of the min-player to be a singleton.


\paragraph{Monotone update} To apply the monotone update in V-learning, we only need to change Line \ref{line:monotone} in Algorithm \ref{algorithm:V}  to 
\begin{equation}
\label{eq:monotone_update}
	V_h(s_h) \setto \min\{H, \tilde{V}_h(s_h),V_h(s_h)\},
\end{equation}
where the only modification is we require the $V$ value estimate never increases, which is why we call it monotone update. 
Intuitively, the reason that this technique would help is in the two-player zero-sum setting $\tilde{V}$ is always an optimistic estimate of the Nash V-value $V^\star$ with high probability (as proved in Lemma \ref{lem:mono_order}). By enforcing this monotone update rule, we guarantee the $V$ value estimate will only move closer to the true Nash V-value $V^\star$ after each update, which  improves the accuracy of our V-value estimates. 
Besides, from a technical perspective, using a $V$-estimate that monotonically approaches $V^\star$ helps avoid some 'averaging' arguments in our analysis that eventually result in the undesired nested mixture of polices.

\paragraph{Output policy} It remains to specify how to compute a Markov output policy. For an arbitrary fixed $(s,h)\in \mathcal{S}\times [H]$, let $t_1$ denote the last time when the value of ${V}_{h,1}(s)$ strictly decreases, and $t_2$ denote the last time when the value of ${V}_{h,2}(s)$ strictly decreases. The output policy $\hat\pi= \hat \pi_1 \times \hat\pi_2$ at $(s,h)$ is defined as  
\begin{equation}\label{eq:monotone_output}
\hat\pi_{h,1}(s):=\sum_{i=1}^{t_2}\alpha_{t_2}^i\pi_{h,1}^{k^i}(s),\quad \hat\pi_{h,2}(s):=\sum_{i=1}^{t_1}\alpha_{t_1}^i\pi_{h,2}^{k^i}(s),
\end{equation}
where $k^i$ denotes the $i^{\rm th}$ time state $s$ is visited at step $h$. Notice that policy $\hat\pi$ is a product Markov policy, since it is history-independent and there is no correlation between the policies of the two players. However, we comment that in order to compute this Markov policy, player $1$ and $2$ need to communicate the indexes of the most recent episodes when their $V$-estimates strictly decrease. As a result, this step is not decentralized. 


\subsection{Theoretical Guarantees} 
We have the following theoretical guarantee showing that V-learning with monotone update enjoys the same sample-efficiency as the original V-learning for finding approximate Nash polices. 

\begin{theorem}
    \label{thm:2p0s_monotone} Suppose subroutine \textsc{Adv\_Bandit\_Update}  satisfies Assumption \ref{ass:external_regret}. For any $\delta \in (0, 1)$ and $K \in \N$, let $\iota = \log(SAT/\delta)$ with $T = KH$ and choose learning rate $\alpha_t$ according to \eqref{eq:hyper_V}, and player $j$ chooses bonus $\{\beta_{t,j}\}_{t=1}^K$ so that $\sum_{i=1}^t\alpha_t^i\beta_{i,j}=\Theta(\AVGReg(A_j, t, \iota)+\sqrt{H^3\iota/t})$ for any $t \in [K]$. Then, with probability at least $1-\delta$, after running Algorithm \ref{algorithm:V} with \emph{monotone update} \eqref{eq:monotone_update} for $K$ episodes,  we have the Markov product policy $\hat{\pi}$ defined by \eqref{eq:monotone_output} satisfies
    \begin{equation*}
        \max_{j\in[2]}[V_{1,j}^{\dag ,\hat{\pi}_{3-j}}(s_1)-V_{1,j}^{\hat{\pi}_1 \times \hat{\pi}_2}(s_1)] \le \cO\left( \frac{HS}{K}\sum_{t=1}^{K/S}\AVGReg(A, t, \iota)+\sqrt{\frac{SH^5\iota}{K}}\right).
    \end{equation*}
  In particular, when instantiate the subroutine \textsc{Adv\_Bandit\_Update} by FTRL (Algorithm~\ref{algorithm:FTRL}), we have
    \begin{equation*}
        \max_{j\in[2]}[V_{1,j}^{\dag ,\hat{\pi}_{3-j}}(s_1)-V_{1,j}^{\hat{\pi}_1 \times \hat{\pi}_2}(s_1)] \le \cO\left(\sqrt{H^5SA\iota/K}+SH^3\iota^2/K \right).
  \end{equation*}
\end{theorem}
In particular, Markov policy $\hat{\pi} = \hat{\pi}_1 \times \hat{\pi}_2$ is  an $\epsilon$-approximate Nash policy if we choose 
  $$
  K \ge \Omega(H^5SA\iota/\epsilon^2+SH^3\iota^2/\epsilon).
  $$
Here, the guarantee is exactly the same as that for vanilla V-learning (Theorem \ref{thm:2p0s_main_result}) except that now we have a Markov policy instead of a nested policy mixture.  
Finally, we remark that the sample complexity above also applies to the single-agent setting (MDPs) by choosing the action set of the min-player to be a singleton. By doing so, we obtain the same sample complexity guarantee for learning $\epsilon$-optimal policy as Theorem \ref{thm:single_main_result}, but the output policy is Markov instead of  a nested policy mixture.









==> prelim_backup.tex <==
%!TEX root = main.tex
\section{Preliminaries} \label{sec:prelim}

We consider multi-player general-sum Markov Games (MG), which are also known as stochastic games in the literature. 
Formally, we denote a general-sum Markov game (general-sum MG) with $m$ players by a tuple $\MG(H, \cS, \{\cA_i\}_{i=1}^m, \P, \{r_i\}_{i=1}^m)$, where $H$, $\cS$ denote the length of each episode and the state space.
 $\cA_i$ denotes the action space for the $i^{\text{th}}$ player and $|\cA_i| = A_i$. We let $\bm{a}:=(a_{1},\cdots,a_{m})$ denote the (tuple of) joint actions of all $m$ players. $\P = \{\P_h\}_{h\in[H]}$ is a collection of transition matrices, so that $\P_h ( \cdot | s, \bm{a}) $ gives the distribution of the next state if actions $\bm{a}$ are taken at state $s$ and step $h$. $r_i = \{r_{h, i}\}_{h\in[H]}$ is a collection of reward functions for the $i^{\text{th}}$ player, so that $r_{h, i}(s, \bm{a})$ gives the reward received by the $i^{\text{th}}$ player if actions $\bm{a}$ are taken at state $s$ and step $h$. 


In each episode of this MG, we start with a \emph{fixed initial state} $s_1$. Then, at each step $h \in [H]$, each player $i$ observes state $s_h \in \cS$, and picks action $a_{h,i}\in\cA_i$ simultaneously. 
After that  each player $i$ receives reward
$r_{h,i}(s_h, \bm{a}_h)$, and the environment transitions to the next state
$s_{h+1}\sim\P_h(\cdot | s_h, \bm{a}_h)$. The episode ends when
$s_{H+1}$ is reached.

% \paragraph{Policy and value function}
% A \emph{policy} $\mu$ of the max-player is a set of $H$ maps $\mu \defeq \big\{ \mu_h: \R \times (\cS \times \cA \times \cB \times \R)^{h-1}\times \cS \rightarrow \Delta_{\cA} \big\}_{h\in [H]}$, from a random number $z$ and a history of length $h$---say $(s_1, a_1, b_1, r_1, \cdots, s_h)$, to a distribution over actions in $\cA$. Here $\Delta_{\cA}$ is the probability simplex over action set $\cA$. Often times, it is sufficient to consider Markov policies, which only depend on the last observed state instead of the entire history and any shared randomness. In symbol, a \emph{Markov policy} $\mu$ of the max-player is a set of $H$ maps $\mu \defeq \big\{ \mu_h: \cS \rightarrow \Delta_{\cA} \big\}_{h\in [H]}$.  Similarly, we can also define the policy and the Markov policy $\nu$ of the min-player,  by replacing the action set $\cA$ in the definitions for the max-player with action set $\cB$.


\paragraph{Markov product policy, value function}
A \emph{Markov} policy $\pi_i$ of player $i$ is a collection of $H$ functions
$\{ \pi_{h,i}: \cS \rightarrow \Delta_{\cA_i} \}_{h\in [H]}$, where each of them maps from a state to a distribution of actions. Here
$\Delta_{\cA_i}$ is the probability simplex over action set
$\cA_i$. 
We denote the product policy of all the players as $\pi:=\pi_1 \times \cdots \times \pi_M$.
We define $V^{\pi}_{h, i}(s)$ as the expected cumulative reward that will be received by the $i^{\text{th}}$ player if starting at state $s$ at step $h$ and all players follow policy $\pi$:
\begin{equation} \label{eq:V_value}
\textstyle V^{\pi}_{h,i}(s) \defeq \E_{\pi}\left[\left.\sum_{h' =
        h}^H r_{h'}(s_{h'}, \bm{a}_{h'}) \right| s_h = s\right].
\end{equation}
We also define $Q^{\pi}_{h,i}:\cS \times \cA\to \mathbb{R}$ to denote $Q$-value function at step $h$ so that
$Q^{\pi}_{h,i}(s, \bm{a})$ gives the cumulative rewards received by player $i$ under policy $\pi$, starting from
$(s, \bm{a})$ at step $h$:
\begin{equation} \label{eq:Q_value}
\textstyle Q^{\pi}_{h,i}(s, \bm{a}) \defeq  \E_{\pi}\left[\left.\sum_{h' = h}^H r_{h'}(s_{h'},  \bm{a}_{h'})
    \right| s_h = s, \bm{a}_h = \bm{a}\right].
\end{equation}
For simplicity, we use notation of operator $\P_h$ so that
$[\P_h V](s, \bm{a}) \defeq \E_{s' \sim \P_h(\cdot|s, \bm{a})}V(s')$ for any value function $V$. We also use notation $[\D_\pi Q](s) \defeq \E_{\bm{a} \sim \pi(\cdot|s)} Q(s, \bm{a})$ for any action-value function $Q$. By definition of value functions, we have the Bellman
equation
\begin{align*}
  Q^{\pi}_{h}(s, \bm{a}) =
  (r_h + \P_h V^{\pi}_{h+1})(s, \bm{a}), \qquad   V^{\pi}_{h}(s)
  =  (\D_{\pi} Q^{\pi}_h)(s) 
\end{align*}
for all $(s, \bm{a}, h) \in \cS \times \cA \times [H]$. We define $V^{\pi}_{H+1}(s) = 0$ for all $s \in \cS_{H+1}$.

\paragraph{General (non-Markovian or non-product) policy}
In certain situations, it is beneficial to consider history-dependent and correlated policies that are not necessarily Markovian or product. A \emph{general policy} $\pi$ is a set of $H$ maps $\pi \defeq \big\{ \pi_{h}: \R \times (\cS \times \cA \times  \R)^{h-1}\times \cS \rightarrow \Delta_{\cA} \big\}_{h\in [H]}$, from a random number $z\in\R$ and a history of length $h$---say $(s_1, \bm{a}_1, r_1, \cdots, s_h)$, to a distribution over the joint action set $\cA$. Here, the random number $z$ is sampled from some underlying distribution $\mathcal{D}$, but may be shared among all steps $h \in [H]$. Given a general policy $\pi$, we use $\pi_i$ to denote the marginalized policy for the $i^{\rm th}$ player, i.e., $\pi_i \defeq \big\{ \pi_{h,i}: \R \times (\cS \times \cA \times  \R)^{h-1}\times \cS \rightarrow \Delta_{\cA_i} \big\}_{h\in [H]}$, and we use $\pi_{-i}$ to denote the joint policy of  all the players except the $i^{\text{th}}$ player, i.e., $\pi_{-i} \defeq \big\{ \pi_{h,-i}: \R \times (\cS \times \cA \times  \R)^{h-1}\times \cS \rightarrow \Delta_{\cA_{-i}} \big\}_{h\in [H]}$ where $\cA_{-i}$ denotes the Cartesian product of the action sets of all players except for player $i$.

For a general policy $\pi$, we can still use the same definitions \eqref{eq:V_value} and  \eqref{eq:Q_value} to define its value functions $V_{h,i}^{\pi}(s)$ and  $Q^{\pi}_{h,i}(s, \bm{a})$ for each $(s,\bm{a},h,i)$ tuple.
 
 
% The value for a pair of policy $(\mu, \nu)$ is defined as the expected cumulative rewards starting from the fixed initial state $s_1$. That is,
% $V_1^{\mu, \nu}(s_1) = \E_{\mu, \nu} []$

% \chijin{This is the definition of Markov policy, define general policy (can be function of all history and random coin here) here.}
% A policy of the max-player is defined as $\mu \defeq \big\{ \mu_h: \cS \rightarrow \Delta_{\cA} \big\}_{h\in [H]}$, and a policy  of the min-player is defined as $\nu \defeq \big\{ \nu_h: \cS \rightarrow \Delta_{\cB} \big\}_{h\in [H]}$. Value and action-value functions of policy $\mu, \nu$ are defined as:
% \begin{align*}
%    \\
% . 
% \end{align*}

\paragraph{Best response}
For any strategy $\pi_{-i}$, there always exists a \emph{best response} of the $i^{\text{th}}$ player, which is a policy $b(\pi_{-i})$ satisfying $V_{h, i}^{b(\pi_{-i}), \pi_{-i}}(s) = \sup_{\pi_i} V_{h, i}^{\pi_i,\pi_{-i}}(s)$ for any $(s, h) \in \cS \times [H]$.
Here the infimum is taken over all possible policies which are not necessarily Markovian, and $\pi_i$ and $\pi_{-i}$ are not correlated during executation. 
To slightly simplify notations, we denote $V_{h, i}^{\dagger, \pi_{-i}} \defeq V_{h, i}^{b(\pi_{-i}), \pi_{-i}}$. The Q-functions of the best response can be defined similarly.
%We further abbreviate the values of Nash equilibrium $V_h^{\mu^\star, \nu^\star}$ and $Q_h^{\mu^\star, \nu^\star}$ as $V_h^{\nash}$ and $Q_h^{\nash}$.
We refer readers to Appendix \ref{app:bellman} for Bellman optimality equations for values of best responses.



\subsection{Learning Objectives}


\paragraph{(Approximate) Nash equilibrium in general-sum MGs.} Our first objective is to find (approximate) Nash equilibria of Markov games. 
Intuitively, a Nash equilibrium gives a solution in which no player has anything to gain by changing only her own policy.


\begin{definition}[Nash equilibrium in general-sum MGs] \label{def:NE}
A product policy $\pi$ is a \textbf{ Nash equilibrium} if $\max_{i\in[m]}{( V_{1,i}^{\dag, \pi_{-i}}-V_{1,i}^{\pi } )}( s_{1} ) = 0$.
\end{definition}
The most well-known special case of multi-player general-sum MGs is two-player zero-sum MG where the payoff of player $1$ is always equal to the negative payoff of player $2$, i.e., $r_1=-r_2$. 
For two-player zero-sum MGs, it is further known (cf.~\citep{filar2012competitive}) that any Nash policy $\pi^\star$
%that are optimal against the best responses of the opponents, in the sense that
%\begin{equation*}
% \textstyle V^{\mu^\star, \dagger}_h(s) = \sup_{\mu}
%      V^{\mu, \dagger}_h(s), 
%      \qquad  V^{\dagger, \nu^\star}_h(s) = \inf_{\nu}
%      V^{\dagger, \nu}_h(s),
%  \qquad \textrm{for all}~(s, h).
%\end{equation*}
%We call these optimal strategies $(\mu^\star,\nu^\star)$ the Nash equilibrium of the Markov game
also satisfies the following minimax equation: 
%\footnote{The minimax theorem here is different from the one for matrix games, i.e. $\max_\phi\min_\psi \phi\trans A\psi = \min_\psi\max_\phi \phi\trans A\psi$ for any matrix $A$, since here $V^{\mu, \nu}_h(s)$ is in general not bilinear in $\mu, \nu$.}
\begin{equation*}
\textstyle   \inf_{\pi_2} V^{\pi_1^\star,\pi_2}_{h,1}(s) = V^{\mu^\star, \nu^\star}_{1,h}(s) = 
-V^{\mu^\star, \nu^\star}_{2,h}(s) =
- \inf_{\pi_1} V^{\pi_1, \pi_2^\star}_{h,2}(s), \qquad \textrm{for all}~(s, h).
\end{equation*}


We can relax the definition of Nash equilibrium by allowing the equality to hold with an $\epsilon$ error, which we denote as $\epsilon$-approximate Nash equilibrium. Formally, 

\begin{definition}[$\epsilon$-approximate Nash equilibrium in general-sum MGs] \label{def:NE_multiplayer}
A product policy $\pi$ is an \textbf{$\epsilon$-approximate Nash equilibrium} if $\max_{i\in[m]}{( V_{1,i}^{\dag, \pi_{-i}}-V_{1,i}^{\pi } )}( s_{1} ) \le \epsilon$.
\end{definition}
% According to Definition \ref{def:NE_multiplayer}, a multiplayer $\epsilon$-approximate Nash equilibrium 

%\begin{definition}[Nash-regret in general-sum MGs]
%  Let $\pi^k$ denote the (product) policy deployed by the algorithm
%  in the $k^{\text{th}}$ episode. After a total of $K$ episodes, the regret is defined as
%  \begin{equation*}
%    \Reg_{\sf Nash}(K) =  \sum_{k=1}^K \max_{i \in [m]}(V_{1,i}^{\dag, \pi_{-i}^k}-V_{1,i}^{\pi^k } )(s_1).
%  \end{equation*}
%\end{definition}


\paragraph{(Approximate) CCE in general-sum MGs.}
% Let us begin with the definition of a CCE policy of a Markov game.
The coarse correlated equilibrium (CCE) is a relaxed version of Nash equilibrium in which we consider general correlated policies instead of product policies. Let $\Acal = \Acal_1 \times \cdots\times \Acal_m$ denote the joint action space.
\begin{definition}
[CCE in general-sum MGs]\label{defn:CCEpolicy}
	A (correlated) policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is a \textbf{CCE} if $\max_{i\in[m]} V^{\dagger,\pi_{-i}}_{1,i}(s_1) \le V^{\pi}_{1,i}(s_1)$.
\end{definition}
Compared with a Nash equilibrium, a CEE is not necessarily a product policy, that is, we may not have $\pi_h(s)\in \Delta_{\Acal_1}\times \cdots\times \Delta_{\Acal_m}$. Similarly, we also define $\epsilon$-approximate  below.
\begin{definition}[$\epsilon$-approximate CCE in general-sum MGs] \label{def:CCE_multiplayer}
A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is an \textbf{$\epsilon$-approximate CCE} if $\max_{i\in[m]}{( V_{1,i}^{\dag, \pi_{-i}}-V_{1,i}^{\pi } )}( s_{1} ) \le \epsilon$.
\end{definition}
%\begin{definition}[CCE-regret in general-sum MGs]
%  Let policy $\pi^k$ denote the (correlated) policy deployed by the algorithm
%  in the $k^{\text{th}}$ episode. After a total of $K$ episodes, the regret is defined as
%  \begin{equation*}
%    \Reg_{\sf CCE}(K) =  \sum_{k=1}^K \max_{i \in [m]}(V_{1,i}^{\dag, \pi_{-i}^k}-V_{1,i}^{\pi^k } )(s_1).
%  \end{equation*}
%\end{definition}
 


\paragraph{(Approximate) CE  in general-sum MGs.}
The correlated equilibrium (CE) is another relaxation of the Nash equilibrium. To define CE, we first introduce the concept of strategy modification:
%\paragraph{Strategy modification.} 
A strategy modification $\phi:=\{ \phi_{h,s}\}_{(h,s)\in[H]\times \cS}$ for player $i$ is a set of $S\times H$ functions from $\Acal_i$ to itself.  Let $\Phi_i$ denote the set of all possible strategy modifications for player $i$.

One can compose a strategy modification $\phi$ with any Markov policy $\pi$ and obtain a  new policy $\phi\circ\pi$ such that when policy $\pi$ chooses to play $\bm{a}:=(a_1,\ldots,a_m)$ at state $s$ and step $h$, policy $\phi\circ\pi$ will play $(a_1,\ldots,a_{i-1},\phi_{h,s}(a_i),a_{i+1},\ldots,a_m)$ instead.
\begin{definition}
[CE in general-sum MGs]\label{defn:CEpolicy}
	A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is a \textbf{CE} if $\max_{i\in[m]}\max_{\phi\in\Phi_i}  V^{\phi\circ\pi}_{1,i}(s_1) \le V^{\pi}_{1,i}(s_1)$.
\end{definition}
Similarly, we have an approximate version of CE.
\begin{definition}[$\epsilon$-approximate CE in Markov games] \label{def:CE_multiplayer}
A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is an \textbf{$\epsilon$-approximate CE} if $\max_{i\in[m]}\max_{\phi\in\Phi_i} (V^{\phi\circ\pi}_{1,i} - V^{\pi}_{1,i})(s_1)\le \epsilon$.
\end{definition}
%\begin{definition}[CE-regret in multiplayer Markov games]
%  Let policy $\pi^k$ denote the policy deployed by the algorithm
%  in the $k^{\text{th}}$ episode. After a total of $K$ episodes, the regret is defined as
%  \begin{equation*}
%    \Reg_{\sf CE}(K) =  \sum_{k=1}^K \max_{i \in [m]}\max_{\phi\in\Phi_i}(\ V^{\phi\circ\pi^k}_{1,i} - V^{\pi^k}_{1,i})(s_1).
%  \end{equation*}
%\end{definition}








==> proof_Q.tex <==
%!TEX root = main.tex


\section{Proof for Nash Q-learning}
\label{app:Q}
In this section, we present proofs for results in Section~\ref{sec:exp-SAB}. 

We denote $V^k, Q^k, \pi^k$ for values and policies \emph{at the beginning} of the $k$-th episode. We also introduce the following short-hand notation
$[\widehat{\P}_{h}^{k}V](s, a, b) := V(s_{h+1}^{k})$.

We will use the following notations several times later: suppose $(s,a,b)$ was taken at the in episodes $k^1,k^2, \ldots $ at the $h$-th step. Since the definition of $k^i$ depends on the tuple $(s,a,b)$ and $h$, we will show the dependence explicitly by writing $k_h^i(s,a,b)$ when necessary and omit it when there is no confusion. We also define $N_{h}^{k}(s,a,b)$ to be the number of times $(s,a,b)$ has been taken \emph{at the beginning} of the $k$-th episode. Finally we denote $n_h^k=N_{h}^{k}\left(  s_{h}^{k},a_{h}^{k},b_{h}^{k} \right) $.


The following lemma is a simple consequence of the update rule in Algorithm~\ref{algorithm:Nash_Q}, which will be used several times later.

\begin{lemma}
   \label{lem:Nash_Q_V}
   Let $t=N_{h}^{k}\left( s,a,b \right) $ and suppose $(s,a,b)$ was previously taken at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. The update rule in Algorithm \ref{algorithm:Nash_Q} is equivalent to the following equations.
   \begin{equation}
      \label{equ:upper-Q-decompose}
   \up{Q}_{h}^{k}(s,a,b)=\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+\up{V}_{h+1}^{k^i}(s_{h+1}^{k^i}) +\beta_i \right]}
   \end{equation}
   \begin{equation}
      \label{equ:lower-Q-decompose}
   \low{Q}_{h}^{k}(s,a,b)=\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+\low{V}_{h+1}^{k^i}(s_{h+1}^{k^i}) -\beta_i \right]}
\end{equation}
\end{lemma}


\subsection{Learning values}
We begin an auxiliary lemma. Some of the analysis in this section is adapted from \cite{jin2018q} which studies Q-learning under the single agent MDP setting.

\begin{lemma}(\citep[Lemma 4.1]{jin2018q})
\label{lem:step_size}
The following properties hold for $\alpha _{t}^{i}$:
% \begin{enumerate}
%    \item $\frac{1}{\sqrt{t}}\le \sum_{i=1}^t{\frac{\alpha _{t}^{i}}{\sqrt{i}}}\le \frac{2}{\sqrt{t}}$.
%    \item $\underset{i\in \left[ t \right]}{\max}\alpha _{t}^{i}\le \frac{2H}{t}$ and $\sum_{i=1}^t{\left( \alpha _{t}^{i} \right) ^2}\le \frac{2H}{t}$ for any $t \ge 1$.
%    \item $\sum_{t=i}^{\infty}{\alpha _{t}^{i}}=1+\frac{1}{H}$ for every $i \ge 1$.
% \end{enumerate}
\begin{enumerate}
\item \label{lem:lr_hoeffding}
$\frac{1}{\sqrt{t}} \le \sum_{i=1}^t \frac{\alpha^i_t}{\sqrt{i}} \le \frac{2}{\sqrt{t}}$ for every $t \ge 1$.
\item \label{lem:lr_property0}
$\max_{i\in[t]} \alpha^i_t \le \frac{2H}{t}$ and $\sum_{i=1}^t (\alpha^i_t)^2 \le \frac{2H}{t}$ for every $t \ge 1$.
\item \label{lem:lr_property}
$\sum_{t=i}^\infty \alpha^i_t = 1 + \frac{1}{H}$ for every $i \geq 1$.
\end{enumerate}
\end{lemma}

We also define $\tilde{\beta} _t:=2\sum_{i=1}^t{\alpha _{t}^{i}\beta_i} \le \cO(\sqrt{H^3\iota/t})$. Now we are ready to prove Lemma~\ref{lem:regret_Nash_Q}.

\begin{proof}[Proof of Lemma~\ref{lem:regret_Nash_Q}]
   We give the proof for one direction and the other direction is similar. For the proof of the first claim, let $t=N_{h}^{k}\left( s,a,b \right) $ and suppose $(s,a,b)$ was previously taken at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. Let $\cF_i$ be the $\sigma$-algebra generated by all the random variables in until the $k^i$-th episode. Then $\{\alpha _{t}^{i}[ ( \widehat{\P}_{h}^{k^i}-\P_h ) V_{h+1}^{\star} ] \left( s,a,b \right)\}_{i=1}^t$ is a martingale differene sequence w.r.t. the filtration $\{\cF_i\}_{i=1}^t$.
    By Azuma-Hoeffding,
   $$
   \left| \sum_{i=1}^t{\alpha _{t}^{i}\left[ \left( \widehat{\P}_{h}^{k^i}-\P_h \right) V_{h+1}^{\star} \right] \left( s,a,b \right)} \right| \le 2H\sqrt{\sum_{i=1}^t{\left( \alpha _{t}^{i} \right) ^2\iota}} \le \tilde{\beta}_t
   $$

Here we prove a stronger version of the first claim by induction: for any $(s,a,b,h,k) \in \cS \times \cA \times \cB \times [H] \times [K]$,
$$ \up{Q}_{h}^{k}(s,a,b) \ge Q^{\star}_h(s,a,b) \ge \low{Q}_{h}^{k}(s,a,b), \,\,\,\, \up{V}_{h}^k(s) \ge V^{\star}_{h}(s) \ge \low{V}_{h}^k(s).
$$

Suppose the guarantee is true for $h+1$, then by the above concentration result, 
    $$
    (\up{Q}_{h}^{k}-Q^{\star}_h)(s,a,b) \ge \alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left( \up{V}_{h+1}^{k^i}-V_{h+1}^{\star} \right) \left( s_{h+1}^{k^i} \right)} \ge 0.
    $$
    
    Also,  
    \begin{align*}
      \up{V}_{h}^k(s) - V^{\star}_{h}(s)=& (\D_{\pi^k_{h}} \up{Q}_{h+1}^k)(s) - \max_{\mu \in \Delta_\cA}\min_{\nu \in \Delta_\cB}(\D_{\mu
      \times \nu} Q_{h+1}^{\star})(s)\\
\ge & \max_{\mu \in \Delta_\cA}
(\D_{\mu \times \nu^k_{h}} \up{Q}_{h}^k)(s) - \max_{\mu \in \Delta_\cA}   (\D_{\mu
\times \nu^k_{h}} Q_{h}^{\star})(s) \ge 0
    \end{align*}
where $\up{Q}_{h}^k (s,a,b) \ge Q_{h}^{\star}(s,a,b)$ has just been proved. The other direction is proved similarly.
% \end{proof}

% Equipped with the above lemmas, we are ready to prove the following Theorem~\ref{lem:bound-phi}, which is the key result to derive the sample complexity guarantee later.
% \begin{theorem}
%    \label{lem:bound-phi}
%    For any $h \in [H]$ and $p \in (0,1)$ , with probability at least $1-p$,
%    $$
%     \sum_{k=1}^K{\left( \up{V}_{h}^{k}-\low{V}_{h}^{k} \right) \left( s_h^k \right)} \le \cO\left( \sqrt{H^4SABT\iota} \right) 
% $$
% As a result,
% \begin{align*}
%     \sum_{k=1}^K{\left( \up{V}_{h}^{k}-V_{h}^{\star} \right) \left( s_h^k \right)} &\le \cO\left( \sqrt{H^4SABT\iota} \right) 
%    \\
%     \sum_{k=1}^K{\left( V_{h}^{\star}-\low{V}_{h}^{k} \right) \left( s_h^k \right)} &\le \cO\left( \sqrt{H^4SABT\iota} \right)   
% \end{align*}
% \end{theorem}

%  \begin{proof}[Proof of Theorem~\ref{lem:bound-phi}]
   Now we continue with the proof of the second claim. Let $t=n_h^k$ and define $\delta _{h}^{k}:=\left( \up{V}_{h}^{k}-\low{V}_{h}^{k} \right) \left( s_{h}^{k} \right)$, then by definition
  \begin{align*}
 \delta _{h}^{k}=&\E_{\left( a,b \right) \sim \pi _{h}^{k}}\left( \up{Q}_{h}^{k}-\low{Q}_{h}^{k} \right) \left( s_{h}^{k},a,b \right) 
 =\left( \up{Q}_{h}^{k}-\low{Q}_{h}^{k} \right) \left( s_{h}^{k},a_{h}^{k},b_{h}^{k} \right) +\zeta_{h}^{k}
 \\
 &\overset{\left( i \right)}{=} \alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\delta _{h+1}^{k_h^i(s_{h}^{k},a_{h}^{k},b_{h}^{k})}}+2\tilde{\beta} _t+\zeta_{h}^{k}
  \end{align*}  
 where $(i)$ is by taking the difference of equation~\eqref{equ:upper-Q-decompose} and equation~\eqref{equ:lower-Q-decompose} and 
 $$
 \zeta_{h}^{k}:=\E_{\left( a,b \right) \sim \pi _{h}^{k}}\left( \up{Q}_{h}^{k}-\low{Q}_{h}^{k} \right) \left( s_{h}^{k},a,b \right) -\left( \up{Q}_{h}^{k}-\low{Q}_{h}^{k} \right) \left( s_{h}^{k},a_{h}^{k},b_{h}^{k} \right)
 $$
 is a martingale difference sequence.

 Taking the summation w.r.t. $k$, we begin with the first two terms, 
   $$
   \sum_{k=1}^K{\alpha _{n_{h}^{k}}^{0}H}=\sum_{k=1}^K{H\mathbb{I}\left\{ n_{h}^{k}=0 \right\}}\le SABH
   $$
   $$
   \sum_{k=1}^K{\sum_{i=1}^{n_{h}^{k}}{\alpha _{n_{h}^{k}}^{i}\delta _{h+1}^{k_h^i\left( s_{h}^{k},a_{h}^{k},b_{h}^{k} \right)}}}\overset{\left( i \right)}{\le} \sum_{k'=1}^K{\delta _{h+1}^{k'}\sum_{i=n_{h}^{k'}+1}^{\infty}{\alpha _{i}^{n_{h}^{k'}}}}\overset{\left( ii \right)}{\le} \left( 1+\frac{1}{H} \right) \sum_{k=1}^K{\delta _{h+1}^{k}}.
   $$
  where $(i)$ is by changing the order of summation and $(ii)$ is by Lemma~\ref{lem:step_size}.

   Plugging them in, 
   \begin{align*}
      \sum_{k=1}^K{\delta _{h}^{k}}\le SABH+\left( 1+\frac{1}{H} \right) \sum_{k=1}^K{\delta _{h+1}^{k}}+\sum_{k=1}^K{\left( 2\tilde{\beta} _{n_{h}^{k}}+\zeta_{h}^{k} \right)}.
   \end{align*}

   Recursing this argument for $h \in [H]$ gives
   $$
   \sum_{k=1}^K{\delta _{1}^{k}}\le eSABH^2+2e\sum_{h=1}^H\sum_{k=1}^K{ \tilde{\beta} _{n_{h}^{k}}}+\sum_{h=1}^H\sum_{k=1}^K{(1+1/H)^{h-1}\zeta_{h}^{k}}
   $$

   By pigeonhole argument,
   $$
   \sum_{k=1}^K{\tilde{\beta} _{n_{h}^{k}}}\le \cO\left( 1 \right) \sum_{k=1}^K{\sqrt{\frac{H^3\iota}{n_{h}^{k}}}}=\cO\left( 1 \right) \sum_{s,a,b}{\sum_{n=1}^{N_{h}^{K}\left( s,a,b \right)}{\sqrt{\frac{H^3\iota}{n}}}}\le \cO\left( \sqrt{H^3SABK\iota} \right) =\cO\left( \sqrt{H^2SABT\iota} \right) 
$$

By Azuma-Hoeffding,
$$
\sum_{h=1}^H{\sum_{k=1}^K{(1+1/H)^{h-1}\zeta _{h}^{k}}}\le e\sqrt{2H^3K\iota}=eH\sqrt{2T\iota}
$$
with high probability. The proof is completed by putting everything together.
 
%  To prove the second claim, by By Lemma~\ref{lem:Nash_q_ULCB}, $
%  \low{V}_{h}^{k}(s)  \le V_{h}^{\star}(s) \le \up{V}_{h}^{k}(s)
%  $. Therefore,
%  $$
%  \sum_{k=1}^K{\left( \up{V}_{h}^{k}-V_{h}^{\star} \right) \left( s_h^k \right)} \le \sum_{k=1}^K{\left( \up{V}_{h}^{k}-\low{V}_{h}^{k} \right) \left( s_h^k \right)} \le \cO\left( \sqrt{H^4SABT\iota} \right) 
%  $$
 \end{proof}

 

 \subsection{Certified policies} \label{app:Q_policy}

 Algorithm~\ref{algorithm:Nash_Q} only learns the value of game but itself cannot give a near optimal policy for each player. In this section, we analyze the certified policy based on the above exploration process (Algorithm~\ref{algorithm:Q-policy}) and prove the sample complexity guarantee. To this end, we need to first define a new group of policies $\hat{\mu}_{h}^{k}$ to facilitate the proof , and $\hat{\nu}_{h}^{k}$ are defined similarly. Notice $\hat{\mu}_{h}^{k}$ is related to $\hat{\mu}$ defined in Algorithm~\ref{algorithm:Q-policy} by $\hat{\mu}=\frac{1}{k}\sum_{i=1}^{k}{\hat{\mu}_{1}^{i}}$.

\begin{algorithm}[h]
   \caption{Policy $\hat{\mu}_{h}^{k}$}
   \label{algorithm:Q-sampling}
   \begin{algorithmic}[1]
      \STATE {\bfseries Initialize:} $k' \setto k$.
      \FOR{step $h'=h,h+1,\dots,H$}
      \STATE Observe $s_{h'}$.
      \STATE Sample $a_{h'} \sim \mu^{k'}_h(s_{h'})$. 
      \STATE Observe $b_{h'}$.
      \STATE $t \setto N^{k'}_h(s_{h'},a_{h'},b_{h'})$.
      \STATE Sample $i$ from $[t]$ with $\P(i)=\alpha^i_t$.
      \STATE $k' \setto k^i_{h'}(s_{h'},a_{h'},b_{h'})$
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

We also define $\hat{\mu}_{h+1}^{k}[s,a,b]$ for $ h \le H-1$, which is na intermediate algorithm only involved in the analysis. The above two policies are related by $\hat{\mu}_{h+1}^{k}\left[ s,a,b \right] =\sum_{i=1}^t{\alpha _{t}^{i}}\hat{\mu}_{h+1}^{k}$ where $t=N_{h}^{k}\left( s,a,b \right) $. $\hat{\nu}_{h+1}^{k}[s,a,b]$ is defined similarly. 

\begin{algorithm}[h]
   \caption{Policy $\hat{\mu}_{h+1}^{k}[s,a,b]$}
   \label{algorithm:Q-sampling-sab}
   \begin{algorithmic}[1]
      \STATE $t \setto N^{k}_{h}(s,a,b)$.
      \STATE Sample $i$ from $[t]$ with $\P(i)=\alpha^i_t$.
      \STATE $k' \setto k^i_h(s,a,b)$
      \FOR{step $h'=h+1,\dots,H$}
      \STATE Observe $s_{h'}$.
      \STATE Sample $a_{h'} \sim \mu^{k'}_h(s_{h'})$. 
      \STATE Observe $b_{h'}$.
      \STATE $t \setto N^{k'}_h(s_{h'},a_{h'},b_{h'})$.
      \STATE Sample $i$ from $[t]$ with $\P(i)=\alpha^i_t$.
      \STATE $k' \setto k^i_{h'}(s_{h'},a_{h'},b_{h'})$
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

Since the policies defined in Algorithm~\ref{algorithm:Q-sampling} and Algorithm~\ref{algorithm:Q-sampling-sab} are non-Markov, many notations for values of Markov policies are no longer valid here. To this end, we need to define the value and Q-value of general policies starting from step $h$, if the general policies starting from the $h$-th step do not depends the history before the $h$-th step. Notice the special case $h=1$ has already been covered in Section~\ref{sec:prelim}. For a pair of general policy $(\mu, \nu)$ which \emph{does not depend} on the hostory before the $h$-th step, we can still use the same definitions \eqref{eq:V_value} and \eqref{eq:Q_value} to define their value $V_h^{\mu, \nu}(s)$ and $Q_h^{\mu, \nu}(s,a,b)$ at step $h$. We can also define the best response $\nu^\dagger(\mu)$ of a general policy $\mu$ as the minimizing policy so that $V_h^{\mu, \dagger}(s) \equiv V_h^{\mu, \nu^\dagger(\mu)}(s) = \inf_{\nu} V_h^{\mu, \nu}(s)$ at step $h$. Similarly, we can define $Q_h^{\mu, \dagger}(s,a,b) \equiv Q_h^{\mu, \nu^\dagger(\mu)}(s,a,b) = \inf_{\nu} Q_h^{\mu, \nu}(s,a,b)$. As before, the best reponse of a general policy is not necessarily Markovian.


It should be clear from the definition of Algorithm~\ref{algorithm:Q-sampling} and Algorithm~\ref{algorithm:Q-sampling-sab} that $\hat{\mu}_{h}^{k}$, $\hat{\nu}_{h}^{k}$, $\hat{\mu}_{h+1}^{k}[s,a,b]$ and $\hat{\nu}_{h+1}^{k}[s,a,b]$ does not depend on the history before step $h$, therefore related value and Q-value functions are well defined for the corresponding steps. Now we can show the policies defined above are indeed certified.

\begin{lemma}
   \label{lem:Nash_q_ULCB_policy}  
   For any $p \in (0,1)$, with probability at least $1-p$, the following holds for any $(s,a,b,h,k) \in \cS \times \cA \times \cB \times [H] \times [K]$,
   $$
   \up{Q}_{h}^{k}(s,a,b) \ge Q_{h}^{\dag ,\hat{\nu}_{h+1}^k[s,a,b]}(s,a,b), \,\,\, \up{V}_{h}^{k}(s) \ge  V_{h}^{\dag ,\hat{\nu}_{h}^{k}}(s)
   $$
   $$
   \low{Q}_{h}^{k}(s,a,b) \le Q_{h}^{\hat{\mu}_{h+1}^k[s,a,b],\dag}(s,a,b), \,\,\, \low{V}_{h}^{k}(s) \le  V_{h}^{\hat{\mu}_{h}^{k},\dag}(s)
   $$
\end{lemma}

 \begin{proof}[Proof of Lemma~\ref{lem:Nash_q_ULCB_policy}]
    We first prove this for $h=H$. 
 \begin{align*}
\up{Q}_{H}^{k}(s,a,b)=&\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_H(s,a,b)+\beta_i \right]}
\\
 \ge & r_H(s,a,b)
 =  Q_{H}^{\dag ,\hat{\nu}_{H+1}^{k}}\left( s,a,b \right)
 \end{align*}
 because $H$ is the last step and
 \begin{align*}
   \up{V}_{H}^{k}(s)=&(\D_{\pi^k_{H}} \up{Q}_{H}^k)(s) 
   \ge  \sup_{\mu \in \Delta_\cA}
   (\D_{\mu \times \nu^k_{H}} \up{Q}_{H}^k)(s)
   \\
    \ge & \sup_{\mu \in \Delta_\cA}
   (\D_{\mu \times \nu^k_{H}} r_{H})(s)
    = V_{H}^{\dag ,\nu_H^k}\left( s \right)
    =  V_{H}^{\dag ,\hat{\nu}_H^k}\left( s \right)
    \end{align*}
    because $\pi_H^k$ is CCE, and by definition $\hat{\nu}_{H}^{k}=\nu_{H}^{k}$.

   Now suppose the claim is true for $h+1$, consider the $h$ case. Consider a fixed tuple $(s,a,b)$ and let $t=N_{h}^{k}\left( s,a,b \right) $. Suppose $(s,a,b)$ was previously taken at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. Let $\cF_i$ be the $\sigma$-algebra generated by all the random variables in until the $k^i$-th episode. Then $\{\alpha _{t}^{i}[ r_h(s,a,b)+V_{h+1}^{\dag ,\hat{\nu}_{h+1}^{k^i}}(s_{h+1}^{k^i}) +\beta_i ]\}_{i=1}^t$ is a martingale differene sequence w.r.t. the filtration $\{\cF_i\}_{i=1}^t$.
   By Azuma-Hoeffding and the definition of $b_i$, 
   $$
  \sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+V_{h+1}^{\dag ,\hat{\nu}_{h+1}^{k^i}}(s_{h+1}^{k^i}) +\beta_i \right]} \ge \sum_{i=1}^t{\alpha _{t}^{i}Q_{h}^{\dag ,\hat{\nu}_{h+1}^{k^i}}(s,a,b)}
   $$
   with high probability. Combining this with the induction hypothesis,

   \begin{align*}
      \up{Q}_{h}^{k}(s,a,b)=&\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+\up{V}_{h+1}^{k^i}(s_{h+1}^{k^i}) +\beta_i \right]}
      \\
      \ge & \sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a,b)+V_{h+1}^{\dag ,\hat{\nu}_{h+1}^{k^i}}(s_{h+1}^{k^i}) +\beta_i \right]}
      \ge \sum_{i=1}^t{\alpha _{t}^{i}Q_{h}^{\dag ,\hat{\nu}_{h+1}^{k^i}}(s,a,b)}
\\
\overset{\left( i \right)}{\ge} & \underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}Q_{h}^{\mu ,\hat{\nu}_{h+1}^{k^i}}(s,a,b)}
= Q_{h}^{\dag ,\hat{\nu}_{h+1}^{k}[s,a,b]}(s,a,b)
\end{align*}
where we have taken the maximum operator out of the summation in $(i)$,which does not increase the sum.

On the other hand,
\begin{align*}
   \up{V}_{h}^{k}(s)=&(\D_{\pi^k_{h}} \up{Q}_{h}^k)(s)
   \overset{\left( i \right)}{\ge} \sup_{\mu \in \Delta_\cA}
   (\D_{\mu \times \nu^k_{h}} \up{Q}_{h}^k)(s) 
   \\
   \overset{\left( ii \right)}{\ge} & \max_{a \in \cA} \E_{b \sim \nu^k_{h} }  Q_{h}^{\dag ,\hat{\nu}_{h+1}^{k}[s,a,b]}(s,a,b)
   = V_{h}^{\dag ,\hat{\nu}_{h}^{k}}(s)
\end{align*}
where $(i)$ is by the definition of CCE and $(ii)$ is the induction hypothesis. The other direction is proved by performing smilar arguments on $\low{Q}_{h}^{k}(s,a,b)$, $Q_{h}^{\hat{\mu}_{h+1}^k[s,a,b],\dag}(s,a,b)$, $\low{V}_{h}^{k}(s)$ and $ V_{h}^{\hat{\mu}_{h}^{k},\dag}(s)$.
 \end{proof}


Finally we give the theoretical guarantee of the policies defined above.

\begin{proof}[Proof of Theorem~\ref{thm:sample_Nash_Q}]
   By lemma~\ref{lem:Nash_q_ULCB_policy}, we have
$$
  \sum_{k=1}^K{\left(V_{1}^{\dag ,\hat{\nu}_{1}^k}-V_{1}^{\hat{\mu}_{1}^k,\dag } \right) \left( s_1 \right)}\le \sum_{k=1}^K{\left(\up{V}_{1}^{k}-\low{V}_{1}^{k} \right) \left( s_1 \right)} 
$$
and Lemma~\ref{lem:regret_Nash_Q} upper bounds this quantity by
$$
\sum_{k=1}^K{\left(V_{1}^{\dag ,\hat{\nu}_{1}^k}-V_{1}^{\hat{\mu}_{1}^k,\dag } \right) \left( s_1 \right)}\le \cO\left( \sqrt{H^4SABT\iota} \right) 
$$

By definition of the induced policy, with probability at least $1-p$, if we run Nash Q-learning (Algorithm~\ref{algorithm:Nash_Q}) for $K$ episodes with 
\begin{equation*}
K \ge \Omega\left(\frac{H^5 SAB\iota}{\epsilon^2}\right),
\end{equation*}
its induced policies $(\hat{\mu}, \hat{\nu})$ (Algorithm \ref{algorithm:Q-policy}) will be $\epsilon$-optimal in the sense $V^{\dagger, \hat{\nu}}_1(s_1) - V^{\hat{\mu}, \dagger}_1(s_1) \le \epsilon$.
\end{proof}
 


==> proof_V.tex <==
%!TEX root = main.tex


\section{Proof for Nash V-learning}
\label{sec:pf_V}


% \begin{algorithm}[t]
% % \setstretch{1.2}
%    \caption{Optimistic Nash V-learning (the max-player version)}
%    \label{algorithm:Nash_V}
%    \begin{algorithmic}[1]
%       \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
%       $\up{V}_{h}(s)\setto H$, $\up{L}_h(s,a) \setto 0$, $N_{h}(s)\setto 0$, $\mu_h(a|s) \setto 1/A$.
%       \FOR{episode $k=1,\dots,K$}
%       \STATE receive $s_1$.
%       \FOR{step $h=1,\dots, H$}
%       \STATE take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $b_h$ from opponent.
%       \STATE observe reward $r_h(s_h, a_h, b_h)$ and next state
%       $s_{h+1}$.
%       \STATE $t=N_{h}(s_h)\setto N_{h}(s_h) + 1$.
%       \STATE $\up{V}_h(s_h) \setto (1-\alpha_t)\up{V}_h(s_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\up{V}_{h+1}(s_{h+1})+\up{\beta}_t)$.
%       \FOR{all $a \in \cA$}
%       \STATE $\up{\ell}^t_h(s_h, a) \setto [H-r_h(s_h, a_h, b_h)-\up{V}_{h+1}(s_{h+1})] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_t]$.
%       \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
%       \ENDFOR
%       \STATE set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_h( s_h, \cdot)]$.
%       \ENDFOR
%       \ENDFOR
%    \end{algorithmic}
% \end{algorithm}


In this section, we present proofs of the results in Section~\ref{sec:exp-SA+B}.
% We begin with the proof of Lemma~\ref{lem:bandit-regret}.
We denote $V^k, \mu^k, \nu^k$ for values and policies \emph{at the beginning} of the $k$-th episode. We also introduce the following short-hand notation
$[\widehat{\P}_{h}^{k}V](s, a, b) := V(s_{h+1}^{k})$.

We will use the following notations several times later: suppose the state $s$ was visited at episodes $k^1,k^2, \ldots $ at the $h$-th step. Since the definition of $k^i$ depends on the state $s$ , we will show the dependence explicitly by writing $k_h^i(s)$ when necessary and omit it when there is no confusion. We also define $N_{h}^{k}(s)$ to be the number of times the state $s$ has been visited \emph{at the beginning} of the $k$-th episode. Finally we denote $n_h^k=N_{h}^{k}\left(  s_{h}^{k} \right) $. Notice the definitions here are different from that in Appendix~\ref{app:Q}.

The following lemma is a simple consequence of the update rule in Algorithm~\ref{algorithm:Nash_V}, which will be used several times later.

\begin{lemma}
   \label{lem:Nash_V_V}
   Let $t=N_{h}^{k}\left( s \right) $ and suppose $s$ was previously visited at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. The update rule in Algorithm \ref{algorithm:Nash_V} is equivalent to the following equations.
   \begin{equation}
      \label{equ:upper-V-decompose}
      \up{V}_{h}^{k}(s)=\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a_h^{k^i},b_h^{k^i})+\up{V}_{h+1}^{k^i}(s_{h+1}^{k^i}) +\up{\beta}_i \right]}
   \end{equation}
   \begin{equation}
      \label{equ:lower-V-decompose}
      \low{V}_{h}^{k}(s)=\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a_h^{k_h^i},b_h^{k_h^i})+\low{V}_{h+1}^{k_h^i}(s_{h+1}^{k_h^i}) -\low{\beta}_i \right]}
\end{equation}
\end{lemma}

\subsection{Missing algorithm details}

We first give Algorithm~\ref{algorithm:Nash_V_min}: the min-player counterpart of Algorithm~\ref{algorithm:Nash_V}. Almost everything is symmetric except the definition of loss function to keep it non-negative.


\begin{algorithm}[t]
   % \setstretch{1.2}
      \caption{Optimistic Nash V-learning (the min-player version)}
      \label{algorithm:Nash_V_min}
      \begin{algorithmic}[1]
         \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
         $\low{V}_{h}(s)\setto 0$, $\low{L}_h(s,b) \setto 0$, $N_{h}(s)\setto 0$, $\nu_h(b|s) \setto 1/B$.
         \FOR{episode $k=1,\dots,K$}
         \STATE receive $s_1$.
         \FOR{step $h=1,\dots, H$}
         \STATE take action $b_h \sim \nu_h(\cdot| s_h)$, observe the action $a_h$ from opponent
         \STATE observe reward $r_h(s_h, a_h, b_h)$ and next state $s_{h+1}$.
         \STATE $t=N_{h}(s_h)\setto N_{h}(s_h) + 1$.
         \STATE $\low{V}_h(s_h) \setto \max\{0,(1-\alpha_t)\low{V}_h(s_h)+ \alpha_t(r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})-\low{\beta}_t)\}$
         \FOR{all $b \in \cB$}
         \STATE $\low{\ell}_h(s_h, b) \setto [r_h(s_h, a_h, b_h)+\low{V}_{h+1}(s_{h+1})] \mathbb{I}\{b_h=b\}/[\nu_h(b_h|s_{h}) +\low{\eta}_t]$.
         \STATE $\low{L}_h( s_h, b)  \setto ( 1-\alpha _t )\low{L}_h( s_h,b ) +\alpha_t \low{\ell}_h(s_h, b)$.
         \ENDFOR
         \STATE set $\nu_h(\cdot |s_h) \propto \exp[-(\low{\eta}_t/\alpha_t) \low{L}_h( s_h, \cdot)]$.
         \ENDFOR
         \ENDFOR
      \end{algorithmic}
   \end{algorithm}
\subsection{Learning values}

We begin with an auxiliary lemma. Some of the analysis in this section is adapted from \cite{jin2018q} which studies Q-learning under the single agent MDP setting.




As usual, we first study learning the value $V^{\star}$ of the Markov game. We begin with an auxiliary lemma, which justifies our choice of confidence bound.

\begin{lemma}
   \label{lem:bandit-regret}
   Let $t=N_{h}^{k}\left( s \right) $ and suppose state $s$ was previously taken at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. Choosing $\up{\eta}_t=\sqrt{\frac{\log A}{At}}$ and $\low{\eta} _t=\sqrt{\frac{\log B}{Bt}}$, with probability $1-p$, for any $(s,h,t) \in \cS \times [H] \times [K]$, there exist a constant $c$ s.t.
$$
\underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i}} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right) }-\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h\left( s,a_{h}^{k^i},b_{h}^{k^i} \right) +\up{V}_{h+1}^{k^i}\left( s_{h+1}^{k^i} \right) \right]}\le c\sqrt{2H^4A\iota /t}
$$
$$
\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h\left( s,a_{h}^{k^i},b_{h}^{k^i} \right) +\low{V}_{h+1}^{k^i}\left( s_{h+1}^{k^i} \right) \right]}-\underset{\nu}{\min}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu _{h}^{k^i} \times \nu} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right)} \le c\sqrt{2H^4B\iota /t}
$$
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:bandit-regret}]
    We prove the first inequality. The proof for the second inequality is similar. We consider thoughout the proof a fixed $(s,h,t) \in \cS \times [H] \times [K]$. Define $\cF_i$ as the $\sigma$-algebra generated by all the random variables before the $k_h^i$-th episode. Then $\{r_h( s,a_{h}^{k^i},b_{h}^{k^i} ) +\up{V}_{h+1}^{k^i}( s_{h+1}^{k^i} )\}_{i=1}^{t}$ is a martingale sequence w.r.t. the filtration $\{\cF_i\}_{i=1}^{t}$. By Azuma-Hoeffding,
$$
\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu _{h}^{k^i} \times \nu _{h}^{k^i}} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right) }-\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h\left( s,a_{h}^{k^i},b_{h}^{k^i} \right) +\up{V}_{h+1}^{k^i}\left( s_{h+1}^{k^i} \right) \right]}\le 2 \sqrt {H^3\iota /t}
$$
So we only need to bound
\begin{equation}\label{eq:regret_definition}
\underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i}} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right) } -\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu _{h}^{k^i} \times \nu _{h}^{k^i}} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right) } := R^\star_t
\end{equation}
where $R^\star_t$ is the weighted regret in the first $t$ times of visiting state $s$, with respect to the optimal policy in hindsight, in the following adversarial bandit problem. The loss function is defined by
$$
l_i(a)=\E_{b \sim \nu _{h}^{k^i}\left( s \right)}\{H-h+1-r_h\left( s,a,b \right) -\P_h\up{V}_{h+1}^{k^i}\left( s,a,b \right)\}
$$
with weight $w_i = \alpha^{i}_t$. We note the weighted regret can be rewrite as $R_t^\star = \sum_{i=1}^t{w_i\left< \mu_h^\star - \mu_h^{k_i}, l_i \right>}$ where $\mu_h^\star$ is argmax for \eqref{eq:regret_definition}, and the loss function satisfies $l_i(a) \in [0, H]$

Therefore, Algorithm~\ref{algorithm:Nash_V} is essentially performing follow the regularized leader (FTRL) algorithm with changing step size for each state to solve this adversarial bandit problem. The policy we are using is $\mu _{h}^{k^i}\left( s,a \right)$ and the optimistic biased estimator
$$
\hat{l}_i(a)= \frac{H-h+1-r_h(s_h^{k^i}, a_h^{k^i}, b_h^{k^i})-\up{V}^{k^i}_{h+1}(s_{h+1}^{k^i})}{\mu _{h}^{k^i}\left( s,a \right) +\up{\eta} _i}\cdot\mathbb{I}\left\{ a_h^{k^i}=a \right\}
$$
is used to handle the bandit feedback.

A more detailed discussion on how to solve the weighted adversarial bandit problem is included in Appendix~\ref{sec:bandit}. Note that $w_i=\alpha_t^i$ is monotonic inscreasing, i.e. $\max _{i\le t}w_i=w_t$. By Lemma \ref{lem:adv-bandit}, we have
% Notice the only difference is we have rescaled the loss to make the presentation in Algorithm~\ref{algorithm:Nash_V} simpler. We make this point in Appendix~\ref{sec:bandit} explicitly by introducing a weight factor $w_i$.
% Now we get bound the regret $R^\star_t$ using lemma~\ref{lem:adv-bandit}. Notice in our problem setting, $w_i=\alpha_t^i$ is monotonic inscreasing. Therefore $\max _{i\le t}w_i=w_t$. As a result,
 \begin{align*}
   R^\star_t &\le 2H\alpha _{t}^{t}\sqrt{At\iota}+\frac{3H\sqrt{A\iota}}{2}\sum_{i=1}^t{\frac{\alpha _{t}^{i}}{\sqrt{i}}}+\frac{1}{2}H\alpha _{t}^{t}\iota +H\sqrt{2\iota \sum_{i=1}^t{\left( \alpha _{t}^{i} \right) ^2}}
\\
&\le 4H^2\sqrt{A\iota /t}+3H\sqrt{A\iota /t}+H^2\iota /t+\sqrt{4H^3\iota /t}
\\
&\le 10H^2\sqrt{A\iota /t}
 \end{align*}
 with probability $1-p/(SHK)$. Finally by a union bound over all $(s,h,t) \in \cS \times [H] \times [K]$, we finish the proof.
\end{proof}

We now prove the following Lemma~\ref{lem:regret_Nash_V}, which is an analoge of Lemma~\ref{lem:regret_Nash_Q} in Nash Q-learning.
\begin{lemma}  \label{lem:regret_Nash_V}
  For any $p\in (0, 1]$, choose hyperparameters as in \eqref{eq:hyper_Nash_V} for large absolute constant $c$ and $\iota = \log (SABT/p)$. Then, with probability at least $1-p$, Algorithm~\ref{algorithm:Nash_V} and \ref{algorithm:Nash_V_min} will jointly provide the following guarantees
  \begin{itemize}
  \item $\up{V}_{h}^{k}(s) \ge V^{\star}_{h}(s) \ge \low{V}_{h}^{k} (s)$ for all $(s, h, k) \in \cS \times [K] \times [H]$.
  \item $(1/K)\cdot \sum_{k=1}^K( \up{V}_{1}^{k}-\low{V}_{1}^{k} ) ( s_1 )  \le \cO\paren{\sqrt{H^6S(A+B)\iota/K}}$.
  \end{itemize}
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:regret_Nash_V}]

   We proof the first claim by backward induction. The claim is true for $h=H+1$. Asumme for any s, $\up{V}_{h+1}^{k}(s) \ge V_{h+1}^{\star}\left( s \right)$, $\low{V}_{h+1}^{k}(s) \le V_{h+1}^{\star}\left( s \right)$. For a fixed $(s,h) \in \cS \times [H]$ and episode $k \in [K]$, let $t=N_{h}^{k}\left( s \right) $ and suppose $s$ was previously visited at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. By Bellman equation,
   \begin{align*}
      V_{h}^{\star}\left( s \right) =&\underset{\mu}{\max}\underset{\nu}{\min}\D_{\mu \times \nu} \left( r_h +\P_h V_{h+1}^{\star} \right) \left( s \right)
      \\
      =&\underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}}\underset{\nu}{\min}\D_{\mu \times \nu} \left( r_h +\P_h V_{h+1}^{\star} \right) \left( s \right)
      \\
      \le& \underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i}} \left( r_h +\P_h V_{h+1}^{\star} \right) \left( s \right)}
      \\
      \le& \underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i}} \left( r_h +\P_h\up{V}_{h+1}^{k^i} \right) \left( s \right)}
   \end{align*}

   Comparing with the decomposition of $\up{V}_{h}^{k}(s)$ in Equation~\eqref{equ:upper-V-decompose} and use Lemma~\ref{lem:bandit-regret}, we can see if $\up{\beta}_t=c\sqrt{AH^4\iota /t}$, then
   $\up{V}_{h}^{k}(s) \ge V_{h}^{\star}\left( s \right)$. Similar by taking $\low{\beta}_t=c\sqrt{BH^4\iota /t}$, we also have $\low{V}_{h}^{k}(s) \le V_{h}^{\star}\left( s \right)$.

   The second cliam is to bound $\delta _{h}^{k}:= \up{V}_{h}^{k}(s_h^k)-\low{V}_{h}^{k}(s_h^k) \ge 0$. Similar to what we have done in Nash Q-learning analysis, taking the difference of Equation~\eqref{equ:upper-V-decompose} and Equation~\eqref{equ:lower-V-decompose},
\begin{align*}
\delta _{h}^{k}=& \up{V}_{h}^{k}(s_h^k)-\low{V}_{h}^{k}(s_h^k)
\\
=&\alpha _{n_h^k}^{0}H+\sum_{i=1}^{n_h^k}{\alpha _{n_h^k}^{i}\left[\left( \up{V}_{h+1}^{k_h^i(s_{h}^{k})}-\low{V}_{h+1}^{k_h^i(s_{h}^{k})} \right)\left( s_{h+1}^{k_h^i(s_{h}^{k})} \right) +\up{\beta}_i+ \low{\beta}_i \right]}
\\
=&\alpha _{n_h^k}^{0}H+\sum_{i=1}^{n_h^k}{\alpha _{n_h^k}^{i}\delta _{h+1}^{k_h^i(s_{h}^{k})}}+\tilde{\beta} _{n_h^k}
\end{align*}
where
$$
\tilde{\beta} _j:=\sum_{i=1}^j{\alpha _{j}^{i}(\up{b}_i+ \low{b}_i}) \le c \sqrt{(A+B)H^4\iota/j}.
$$

Taking the summation w.r.t. $k$, we begin with the first two terms,
$$
\sum_{k=1}^K{\alpha _{n_{h}^{k}}^{0}H}=\sum_{k=1}^K{H\mathbb{I}\left\{ n_{h}^{k}=0 \right\}}\le SH
$$
$$
\sum_{k=1}^K{\sum_{i=1}^{n_{h}^{k}}{\alpha _{n_{h}^{k}}^{i}\delta _{h+1}^{k_h^i\left( s_{h}^{k} \right)}}}\overset{\left( i \right)}{\le} \sum_{k'=1}^K{\delta _{h+1}^{k'}\sum_{i=n_{h}^{k'}+1}^{\infty}{\alpha _{i}^{n_{h}^{k'}}}}\overset{\left( ii \right)}{\le} \left( 1+\frac{1}{H} \right) \sum_{k=1}^K{\delta _{h+1}^{k}}.
$$
where $(i)$ is by changing the order of summation and $(ii)$ is by Lemma~\ref{lem:step_size}. Putting them together,

\begin{align*}
    \sum_{k=1}^K{\delta _{h}^{k}}=&\sum_{k=1}^K{\alpha _{n_{h}^{k}}^{0}H}+\sum_{k=1}^K{\sum_{i=1}^{n_{h}^{k}}{\alpha _{n_{h}^{k}}^{i}\delta _{h+1}^{k_h^i\left( s_{h}^{k} \right)}}}+\sum_{k=1}^K{\tilde{\beta} _{n_{h}^{k}}}
\\
\le& HS+\left( 1+\frac{1}{H} \right) \sum_{k=1}^K{\delta _{h+1}^{k}}+\sum_{k=1}^K{\tilde{\beta} _{n_{h}^{k}}}
\end{align*}
Recursing this argument for $h \in [H]$ gives
   $$
   \sum_{k=1}^K{\delta _{1}^{k}}\le eSH^2+e\sum_{h=1}^H\sum_{k=1}^K{\tilde{\beta} _{n_{h}^{k}}}
   $$

   By pigeonhole argument,
   \begin{align*}
   \sum_{k=1}^K{\tilde{\beta} _{n_{h}^{k}}}&\le \cO\left( 1 \right) \sum_{k=1}^K{\sqrt{\frac{(A+B)H^4\iota}{n_{h}^{k}}}}
   =\cO\left( 1 \right) \sum_{s}{\sum_{n=1}^{n_{h}^{K}\left( s \right)}{\sqrt{\frac{(A+B)H^4\iota}{n}}}}\\
   &\le \cO\left( \sqrt{H^4S(A+B)K\iota} \right) =\cO\left( \sqrt{H^3S(A+B)T\iota} \right)
   \end{align*}

Expanding this formula repeatedly and apply pigeonhole argument we have
\begin{equation*}
\sum_{k=1}^K{[\up{V}_{h}^{k}-\low{V}_{h}^{k}](s_1)} \le \cO(\sqrt{H^5S(A+B)T\iota}).
\end{equation*}
which finishes the proof.
% As a result,
% \begin{align*}
%    \sum_{k=1}^K{\left( \up{V}_{h}^{k}-V_{h}^{\star} \right) \left( s_h^k \right)} &\le \cO\left( \sqrt{H^5S(A+B)T\iota} \right)
%   \\
%    \sum_{k=1}^K{\left( V_{h}^{\star}-\low{V}_{h}^{k} \right) \left( s_h^k \right)} &\le \cO\left( \sqrt{H^5S(A+B)T\iota} \right)
% \end{align*}
\end{proof}

\subsection{Certified policies}

% \begin{algorithm}[h]
%    \caption{Policy $\hat{\mu}_{h}^{k}$}
%    \label{algorithm:V-sampling}
%    \begin{algorithmic}[1]
%       \STATE {\bfseries Initialize:} $k' \setto k$.
%       \FOR{step $h'=h,h+1,\dots,H$}
%       \STATE Observe $s_{h'}$.
%       \STATE $t \setto N^{k'}_h(s_{h'})$.
%       \STATE Sample $i$ from $[t]$ with $\P(i)=\alpha^i_t$.
%       \STATE $k' \setto k^i_{h'}(s_{h'})$
%       \STATE Sample $a_{h'} \sim \mu^{k'}_h(s_{h'})$.
%       \ENDFOR
%    \end{algorithmic}
% \end{algorithm}


As before, we construct a series of new policies  $\hat{\mu}_{h}^{k}$ in Algorithm~\ref{algorithm:V-sampling}. Notice $\hat{\mu}_{h}^{k}$ is related to $\hat{\mu}$ defined in Algorithm~\ref{algorithm:V-policy} by $\hat{\mu}=\frac{1}{k}\sum_{i=1}^{k}{\hat{\mu}_{1}^{i}}$. Also we need to consider value and Q-value functions of general policies which \emph{does not depend} on the hostory before the $h$-th step. See Appendix~\ref{app:Q_policy} for details. Again, we can show the policies defined above are indeed certified.





\begin{lemma}
   \label{lem:v_ULCB_policy}
   For any $p \in (0,1)$, with probability at least $1-p$, the following holds for any $(s,a,b,h,k) \in \cS \times \cA \times \cB \times [H] \times [K]$,
   $$
 \up{V}_{h}^{k}(s) \ge  V_{h}^{\dag ,\hat{\nu}_{h}^{k}}(s), \,\,\,
 \low{V}_{h}^{k}(s) \le  V_{h}^{\hat{\mu}_{h}^{k},\dag}(s)
   $$
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:v_ULCB_policy}]
    We prove one side by induction and the other side is similar. The claim is trivially satisfied for $h=H+1$. Suppose it is ture for $h+1$, consider a fixed state $s$. Let $t=N_{h}^{k}\left( s \right) $ and suppose $s$ was previously visited at episodes $k^1,\ldots, k^t < k$ at the $h$-th step. Then using Lemma~\ref{lem:Nash_V_V},
\begin{align*}
   \up{V}_{h}^{k}(s)&=\alpha _{t}^{0}H+\sum_{i=1}^t{\alpha _{t}^{i}\left[ r_h(s,a_h^{k^i},b_h^{k_h^i})+\up{V}_{h+1}^{k^i}(s_{h+1}^{k^i}) +\up{\beta}_i \right]}
\\
&\overset{\left( i \right)}{\ge} \underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i} }\left( r_h +\P_h\up{V}_{h+1}^{k^i} \right)\left( s \right)}
\\
&\overset{\left( ii \right)}{\ge} \underset{\mu}{\max}\sum_{i=1}^t{\alpha _{t}^{i}\D_{\mu \times \nu _{h}^{k^i} }\left( r_h +\P_h V_{h+1}^{\dag ,\hat{\nu}_{h+1}^{k^i}} \right)\left( s \right)}
\\
&=V_{h}^{\dag ,\hat{\nu}_{h}^{k}}(s)
\end{align*}
where $(i)$ is by using Lemma~\ref{lem:bandit-regret} and the definition of $\up{\beta}_i$, and $(ii)$ is by induction hypothesis.
\end{proof}


Equipped with the above lemmas, we are now ready to prove Theorem~\ref{thm:sample_Nash_V}.

\begin{proof}[Proof of Theorem~\ref{thm:sample_Nash_V}]
   By lemma~\ref{lem:v_ULCB_policy}, we have
$$
  \sum_{k=1}^K{\left(V_{1}^{\dag ,\hat{\nu}_{1}^k}-V_{1}^{\hat{\mu}_{1}^k,\dag } \right) \left( s_1 \right)}\le \sum_{k=1}^K{\left(\up{V}_{1}^{k}-\low{V}_{1}^{k} \right) \left( s_1 \right)}
$$
and Lemma~\ref{lem:regret_Nash_V} upper bounds this quantity by
$$
   \sum_{k=1}^K{\left(V_{1}^{\dag ,\hat{\nu}_{1}^k}-V_{1}^{\hat{\mu}_{1}^k,\dag } \right) \left( s_1 \right)}\le \cO\left( \sqrt{H^5S(A+B)T\iota} \right)
$$

By definition of the induced policy, with probability at least $1-p$, if we run Nash V-learning (Algorithm~\ref{algorithm:Nash_V}) for $K$ episodes with
\begin{equation*}
K \ge \Omega\left(\frac{H^6 S(A+B)\iota}{\epsilon^2}\right),
\end{equation*}
its induced policies $(\hat{\mu}, \hat{\nu})$ (Algorithm \ref{algorithm:V-policy}) will be $\epsilon$-optimal in the sense $V^{\dagger, \hat{\nu}}_1(s_1) - V^{\hat{\mu}, \dagger}_1(s_1) \le \epsilon$.
\end{proof}


==> proof_lower.tex <==
%!TEX root = main.tex


\section{Proofs of Hardness for Learning the Best Responses}
\label{appendix:proof-lower}
\label{appendix:proof-lower-bound-coupled}

In this section we give the proof of Theorem~\ref{theorem:lower-bound-best-response}, and Corollary~\ref{cor:lower-bound-coupled}. Our proof is inspired by a computational hardness result for adversarial MDPs in~\citep[Section 4.2]{yadkori2013online}, which constructs a family of adversarial MDPs that are computationally as hard as an agnostic parity learning problem.

Section \ref{app:hard_instance}, \ref{app:series_hard_pbs}, \ref{app:hard_together} will be devoted to prove Theorem \ref{theorem:lower-bound-best-response}, while Corollary \ref{cor:lower-bound-coupled} is proved in Section \ref{sec:adversarial_proof}.
Towards proving Theorem \ref{theorem:lower-bound-best-response}, we will:
\begin{itemize}
  \item (Section \ref{app:hard_instance}) Construct a Markov game. 
  \item (Section \ref{app:series_hard_pbs}) Define a series of problems where a solution in problem implies another.
  \item (Section \ref{app:hard_together}) Based on the believed computational hardness of learning paries with noise (Conjecture~\ref{conj:hardness}), we conclude that finding the best response of non-Markov policies is computationally hard.
\end{itemize}



\subsection{Markov game construction}
\label{app:hard_instance}
We now describe a Markov game inspired the adversarial MDP in \citep[Section 4.2]{yadkori2013online}.
We define a Markov game in which we have $2H$ states, $\left\{ i_0,i_1 \right\} _{i=2}^{H}$, $1_0$ (the initial state) and $\bot$ (the terminal state)\footnote{In \cite{yadkori2013online} the states are denoted by $\left\{ i_a,i_b \right\} _{i=2}^{H}$ instead. Here we slightly change the notation to make it different from the notation of the actions}. In each state the max-player has two actions $a_0$ and $a_1$, while the min-player has two actions $b_0$ and $b_1$. The transition kernel is deterministic and the next state for steps $h\le H-1$ is defined in Table~\ref{table:parity-learning-transition}:
% \begin{table}[h]
%   \centering
%   \begin{tabular}{l|l|l|l|l}
%   State/Action & $(a_0,b_0)$ & $(a_0,b_1)$ & $(a_1,b_0)$ & $(a_1,b_1)$ \\ \hline
%   $i_0$             & $(i+1)_0$   & $(i+1)_0$   & $(i+1)_0$   & $(i+1)_1$   \\ \hline
%   $i_1$             & $(i+1)_1$   & $(i+1)_0$   & $(i+1)_1$   & $(i+1)_1$  
%   \end{tabular}
%   \caption{Transition kernel of the hard instance for coupled players.}
% \end{table}

\begin{table}[h]
  \centering
  \begin{tabular}{|c|c|c|c|c|} \hline
    State/Action & $(a_0,b_0)$ & $(a_0,b_1)$ & $(a_1,b_0)$ & $(a_1,b_1)$ \\ \hline
    $i_0$             & $(i+1)_0$   & $(i+1)_0$   & $(i+1)_0$   & $(i+1)_1$   \\ \hline
    $i_1$             & $(i+1)_1$   & $(i+1)_0$   & $(i+1)_1$   & $(i+1)_1$  \\\hline
  \end{tabular}
  \caption{Transition kernel of the hard instance.
  }
  \label{table:parity-learning-transition}
\end{table}
At the $H$-th step, i.e. states $H_0$ and $H_1$, the next state is always $\bot$ regardless of the action chosen by both players. The reward function is always $0$ except at the $H$-th step. The reward is determined by the action of the min-player, defined by 
\begin{table}[h]
  \centering
  \begin{tabular}{|c|c|c|} \hline
    State/Action & $(\cdot,b_0)$ & $(\cdot,b_1)$ \\ \hline
  $H_0$             & $1$           & $0$           \\ \hline
  $H_1$             & $0$           & $1$          \\ \hline
  \end{tabular}
  \caption{Reward of the hard instance.}
\end{table}

At the beginning of every episode $k$, both players pick their own policies $\mu_k$ and $\nu_k$, and execute them throughout the episode. The min-player can possibly pick her policy $\nu_k$ adaptive to all the observations in the earlier episodes. The only difference from the standard Markov game protocol is that the actions of the min-player except the last step will be revealed at the beginning of each episode, to match the setting in agnostic learning parities (Problem 2 below). Therefore we are actually considering a easier problem (for the max-player) and the lower bound naturally applies.

\subsection{A series of computationally hard problems}
\label{app:series_hard_pbs}
We first introduce a series of problems and then show how the reduction works.

\paragraph{Problem 1} The max-player $\epsilon$-approximates the best reponse for any general policy $\nu$ in the Markov game defined in Appendix~\ref{app:hard_instance} with probability at least $1/2$, in $\poly(H,1/\epsilon)$ time.




\paragraph{Problem 2} Let $x=\left( x_1,\cdots ,x_n \right) $ be a vector in $\left\{ \text{0,}1 \right\} ^n$, $T\subseteq \left[ n \right]$ and $0< \alpha < 1/2$.The parity of $x$ on $T$ is the boolean function $\phi _T\left( x \right) =\oplus _{i\in T}x_i$. In words, $\phi _T\left( x \right)$ outputs $0$ if the number of
ones in the subvector $(x_i)_{i \in T}$ is even and $1$ otherwise. A uniform query oracle for
this problem is a randomized algorithm that returns a random uniform vector $x$, as
well as a noisy classification $f(x)$ which is equal to $\phi_T(x)$ w.p. $\alpha$ and $1 -\phi_T(x)$ w.p. $1-\alpha$. All examples returned by the oracle are independent. The learning parity with noise problem consists in designing an algorithm with
access to the oracle such that,
\begin{itemize}
  \item (\textbf{Problem 2.1}) w.p at least $1/2$, find a (possibly random) function $h: \{0, 1\}^n \rightarrow \{0, 1\}$ satisy $\E_h P_x[h(x) \neq \phi_T(x)] \le \epsilon$, in $\poly(n ,1/\epsilon)$ time.
  \item (\textbf{Problem 2.2}) w.p at least $1/4$, find $h: \{0, 1\}^n \rightarrow \{0, 1\}$ satisy $P_x[h(x) \neq \phi_T(x)] \le \epsilon$, in $\poly(n ,1/\epsilon)$ time.
  \item  (\textbf{Problem 2.3}) w.p at least $1-p$, find $h: \{0, 1\}^n \rightarrow \{0, 1\}$ satisy $P_x[h(x) \neq \phi_T(x)] \le \epsilon$, in $\poly(n ,1/\epsilon, 1/p)$ time.
\end{itemize}

We remark that Problem 2.3 is the formal definition of learning parity with noise \citep[Definition 2]{mossel2005learning}, which is conjectured to be computationally hard in the community (see also Conjecture \ref{conj:hardness}).

  
\paragraph{Problem 2.3 reduces to Problem 2.2}

Step 1: Repeatly apply algorithm for Problem 2.2 $\ell$ times to get $h_1,\dots,h_\ell$ such that $\min_i P_x[h_i(x)\neq \phi_T(x)] \le \epsilon$ with probability at least $1-(3/4)^\ell$. This costs $\poly(n, \ell, 1/\epsilon)$ time. Let $i_\star = \argmin_i {\rm err}_i$ where ${\rm err}_i = P_x[h_i(x)\neq \phi_T(x)]$.

Step 2: Construct estimators using $N$ additional data ${(x^{(j)},y^{(j)})}_{j=1}^N$,
\begin{equation*}
  \hat{\rm err}_i \defeq \frac{\frac{1}{N} \sum_{j=1}^N \mathbb{I}\{ h_i(x^{(j)}) \neq y^{(j)} \} - \alpha}{1-2\alpha}.
\end{equation*}
Pick $\hat{i} = \argmin_i \hat{\rm err}_i$. When $N\ge \log(1/p)/\epsilon^2$, with probability at least $1-p/2$, we have
\begin{equation*}
  \max_i \left| \hat{\rm err}_i - {\rm err}_i \right| \le \frac{\epsilon}{1-2\alpha}.
\end{equation*}
This means that
\begin{equation*}
  {\rm err}_{\hat{i}} \le \hat{\rm err}_{\hat{i}} + \frac{\epsilon}{1-2\alpha} \le \hat{\rm err}_{i_\star} + \frac{\epsilon}{1-2\alpha} \le {\rm err}_{i_\star} + \frac{2\epsilon}{1-2\alpha} \le O(1)\epsilon.
\end{equation*}
This step uses $\poly(n, N, \ell)=\poly(n, 1/\epsilon, \log(1/p), \ell)$ time.

Step 3: Pick $\ell=\log(1/p)$, we are guaranteed that good events in step 1 and step 2 happen with probability $\ge 1-p/2$ and altogether happen with probability at least $1-p$. The total time used is $\poly(n, 1/\epsilon, \log(1/p))$. Note better dependence on $p$ than required.


\paragraph{Problem 2.2 reduces to Problem 2.1:}
If we have an algorithm that gives $\E_{h \sim \cD} P_x[h(x) \neq \phi_T(x)] \le \epsilon$ with probability $1/2$. Then if we sample $\hat{h} \sim \cD$, by Markov's inequality, we have with probability $\ge 1/4$ that 
\begin{equation*}
P_x[\hat{h}(x) \neq \phi_T(x)] \le 2\epsilon
\end{equation*}


\paragraph{Problem 2.1 reduces to Problem 1:}
Consider the Markov game constructed above with $H-1=n$. The only missing piece we fill up here is the policy $\nu$ of the min-player, which is constructed as following. The min-player draws a sample $(x,y)$ from the uniform query oracle, then taking action $b_0$ at the step $h \le H-1$ if $x_h=0$ and $b_1$ otherwise. For the $H$-th step, the min-player take action $b_0$ if $y=0$ and $b_1$ otherwise. Also notice the policy $\hat{\mu}$ of the max-player can be descibed by a set $\hat{T} \subseteq [H]$ where he takes action $a_1$ at step $h$ if $h $ and $a_0$ otherwise. As a result, the max-player receive non-zero result iff $\phi_{\hat{T}}(x)=y$.



In the Markov game, we have $V_1^{\hat{\mu}, \nu}(s_1) = \P(\phi_{\hat{T}}(x)=y)$. As a result, the optimal policy $\mu^{*}$ corresponds to the true parity set $T$. As a result,
$$
(V_1^{\dagger, \nu}-V_1^{\hat{\mu}, \nu})(s_1)=\P_{x, y}(\phi_T(x) = y) - \P_{x, y}(\phi_{\hat{T}}(x) = y) \le \epsilon
$$
by the $\epsilon$-approximation guarantee.

Also notice
\begin{align*}
 \P_{x, y}(\phi_{\hat{T}}(x) \neq y) - \P_{x, y}(\phi_{T}(x) \neq y)
 =& (1-\alpha) \P_x(\phi_{\hat{T}}(x) \neq \phi_{T}(x)) + \alpha \P_x(\phi_{\hat{T}}(x) = \phi_{T}(x)) - \alpha\\
 =& (1-2\alpha) \P_x(\phi_{\hat{T}}(x) \neq \phi_{T}(x))
\end{align*}

This implies:

\begin{equation*}
\P_x(\phi_{\hat{T}}(x) \neq \phi_{T}(x)) \le \frac{\epsilon}{1-2\alpha}
\end{equation*}

\subsection{Putting them together}
\label{app:hard_together}
So far, we have proved that Solving Problem 1 implies solving Problem 2.3, where Problem 1 is the problem of learning $\epsilon$-approximate best response in Markov games (the problem we are interested in), and Problem 2.3 is precisely the problem of learning parity with noise \cite{mossel2005learning}. This concludes the proof.


\subsection{Proofs of Hardness Against Adversarial Opponents}
\label{sec:adversarial_proof}
Corollary~\ref{cor:lower-bound-coupled} is a direct consequence of Theorem~\ref{theorem:lower-bound-best-response}, as we will show now.

\begin{proof}[Proof of Corollary~\ref{cor:lower-bound-coupled}]
We only need to prove a polynomial time no-regret algorithm also learns the best response in a Markov game where the min-player following non-Markov policy $\nu$. Then the no-regret guarantee implies,
$$
   V^{\dagger, \nu}_{1}
  (s_1) -\frac{1}{K}  \sum_{k=1}^K V^{\mu^k, \nu}_{1} (s_1) \le {\rm poly}(S, H, A, B)K^{-\delta}
$$
where $\mu_k$ is the policy of the max-player in the $k$-th episode. If we choose $\hat{\mu}$ uniformly randomly from $\set{\mu_k}_{k=1}^K$, then 
$$ V^{\dagger, \nu}_{1}
(s_1) - V^{\hat{\mu}, \nu}_{1}
(s_1)  \le {\rm poly}(S, H, A, B)K^{-\delta}.
$$

Choosing $\epsilon = {\rm poly}(S, H, A, B)K^{-\delta}$, $K={\rm poly}(S, H, A, B, 1/\epsilon)$ and the running time of the no-regret algorithm is still ${\rm poly}(S, H, A, B, 1/\epsilon)$ to learn the $\epsilon$-approximate best response.

To see that the Corollary~\ref{cor:lower-bound-coupled} remains to hold for policies that are Markovian in each episode and non-adaptive, we can take the hard instance in Theorem~\ref{theorem:lower-bound-best-response} and let $\nu^k$ denote the min-player's policy in the $k$-th episode. Note that each $\nu^k$ is Markovian and non-adaptive on the observations in previous episodes. If there is a polynomial time no-regret algorithm against such $\set{\nu^k}$, then by the online-to-batch conversion similar as the above, the mixture of $\set{\mu_k}_{k=1}^K$ learns a best response against $\nu$ in polynomial time.


\end{proof}



==> property.tex <==
%!TEX root = main.tex


\section{Bellman Equations for Markov Games}
\label{app:bellman}

In this section, we present the Bellman equations for different types of values in Markov games.

\paragraph{Fixed policies.} For any pair of Markov policy $(\mu, \nu)$, by definition of their values in \eqref{eq:V_value} \eqref{eq:Q_value}, we have the following Bellman equations:
\begin{align*}
  Q^{\mu, \nu}_{h}(s, a, b) =  (r_h + \P_h V^{\mu, \nu}_{h+1})(s, a, b), \qquad   
  V^{\mu, \nu}_{h}(s)  =  (\D_{\mu_h\times\nu_h} Q^{\mu, \nu}_h)(s) 
\end{align*}
for all $(s, a, b, h) \in \cS \times \cA \times \cB \times [H]$, where $V^{\mu, \nu}_{H+1}(s) = 0$ for all $s \in \cS_{H+1}$.

\paragraph{Best responses.} For any Markov policy $\mu$ of the max-player, by definition, we have the following Bellman equations for values of its best response:
\begin{align*}
Q^{\mu, \dagger}_{h}(s, a, b) = (r_h + \P_h V^{\mu, \dagger}_{h+1})(s, a, b), \qquad
V^{\mu, \dagger}_{h}(s) = \inf_{\nu \in \Delta_{\cB}} (\D_{\mu_h \times \nu} Q^{\mu, \dagger}_h)(s),
\end{align*}
for all $(s, a, b, h) \in \cS \times \cA \times \cB \times [H]$, where $V^{\mu, \dagger}_{H+1}(s) = 0$ for all $s \in \cS_{H+1}$.

Similarly, for any Markov policy $\nu$ of the min-player, we also have the following symmetric version of Bellman equations for values of its best response:
\begin{align*}
Q^{\dagger, \nu}_{h}(s, a, b) =  (r_h + \P_h V^{\dagger, \nu}_{h+1})(s, a, b), \qquad 
V^{\dagger, \nu}_{h}(s) = \sup_{\mu \in \Delta_{\cA}} (\D_{\mu \times \nu_h} Q^{\dagger, \nu}_h)(s).
\end{align*}
for all $(s, a, b, h) \in \cS \times \cA \times \cB \times [H]$, where $V^{\dagger, \nu}_{H+1}(s) = 0$ for all $s \in \cS_{H+1}$.

\paragraph{Nash equilibria.} Finally, by definition of Nash equilibria in Markov games, we have the following Bellman optimality equations:
\begin{align*}
Q^{\nash}_{h}(s, a, b) = &  (r_h + \P_h V^{\nash}_{h+1})(s, a, b) \\
V^{\nash}_{h}(s) =&
  \sup_{\mu \in \Delta_{\cA}}\inf_{\nu \in \Delta_{\cB}} (\D_{\mu \times \nu} Q^{\nash}_h)(s)
  = \inf_{\nu \in \Delta_{\cB}}\sup_{\mu \in \Delta_{\cA}} (\D_{\mu \times \nu} Q^{\nash}_h)(s).
\end{align*}
for all $(s, a, b, h) \in \cS \times \cA \times \cB \times [H]$, where $V^{\nash}_{H+1}(s) = 0$ for all $s \in \cS_{H+1}$.



% \subsection{Q-learning}
% Q-learning \citep{watkins1989learning} is a classical model-free algorithm for learning Markov decision process. It is one of the most popular algorithms in the literature of reinforcement learning. Nash Q-learning is firstly proposed in \cite{hu2003nash}, which adapted the classical Q-learning to solve multi-agent Markov games. Nash Q-learning features two most important steps:
% \begin{enumerate}
%  \item an online incremental update of $Q$-value functions with parameter $\alpha$.
%  \begin{equation*}
%  Q_h(s_h, a_h, b_h) \setto (1-\alpha)Q_h(s_h, a_h, b_h)+ \alpha(r_h+V_{h+1}(s_{h+1}))
%  \end{equation*}
%  where tuple $(s_h, a_h, b_h, r_h, s_{h+1})$ is the observation in the current step.
%  \item a computation of greedy policies per step.
%  \begin{equation*}
%  (\mu_h(\cdot|s), \nu_h(\cdot|s)) \leftarrow \arg \max_{\mu \in \Delta_{\cA}}\min_{\nu \in \Delta_{\cB}} (\D_{\mu \times \nu} Q_h)(s)
%   = \arg \min_{\nu \in \Delta_{\cB}}\max_{\mu \in \Delta_{\cA}} (\D_{\mu \times \nu} Q_h)(s)
%  \end{equation*}
% \end{enumerate}
 

\section{Properties of Coarse Correlated Equilibrium}
\label{app:CCE}
% \subsection{CCE}
Recall the definition for CCE in our main paper \eqref{eq:CCE}, we restate it here after rescaling. For any pair of matrix $P, Q \in [0, 1]^{n\times m}$, the subroutine $\textsc{CCE}(P, Q)$ returns a distribution $\pi \in \Delta_{n \times m}$ that satisfies:
\begin{align}
\E_{(a, b) \sim \pi} P(a, b) \ge& \max_{a^\star} \E_{(a, b) \sim \pi} P(a^\star, b)  \label{eq:constraints_CCE}\\
\E_{(a, b) \sim \pi} Q(a, b) \le& \min_{b^\star} \E_{(a, b) \sim \pi} Q(a, b^\star) \nonumber
\end{align}
We make three remarks on CCE. First, a CCE always exists since a Nash equilibrium for a general-sum game with payoff matrices $(P, Q)$ is also a CCE defined by $(P, Q)$, and a Nash equilibrium always exists. Second, a CCE can be efficiently computed, since above constraints \eqref{eq:constraints_CCE} for CCE can be rewritten as $n+m$ linear constraints on $\pi \in \Delta_{n \times m}$, which can be efficiently resolved by standard linear programming algorithm. Third, a CCE in general-sum games needs not to be a Nash equilibrium. However, a CCE in zero-sum games is guaranteed to be a Nash equalibrium.
\begin{proposition}\label{prop:CCE}
Let $\pi = \textsc{CCE}(Q, Q)$, and $(\mu, \nu)$ be the marginal distribution over both players' actions induced by $\pi$. Then $(\mu, \nu)$ is a Nash equilibrium for payoff matrix $Q$.
\end{proposition}

\begin{proof}[Proof of Proposition \ref{prop:CCE}]
Let $N^\star$ be the value of Nash equilibrium for $Q$. Since $\pi = \textsc{CCE}(Q, Q)$, by definition, we have:
\begin{align*}
\E_{(a, b) \sim \pi} Q(a, b) \ge& \max_{a^\star} \E_{(a, b) \sim \pi} Q(a^\star, b) = \max_{a^\star} \E_{b \sim \nu} Q(a^\star, b) \ge N^\star\\
\E_{(a, b) \sim \pi} Q(a, b) \le& \min_{b^\star} \E_{(a, b) \sim \pi} Q(a, b^\star) =\min_{b^\star} \E_{a \sim \mu} Q(a, b^\star) \le N^\star
\end{align*}
This gives:
\begin{equation*}
\max_{a^\star} \E_{b \sim \nu} Q(a^\star, b) = \min_{b^\star} \E_{a \sim \mu} Q(a, b^\star) = N^\star
\end{equation*}
which finishes the proof.
\end{proof}
Intuitively, a CCE procedure can be used in Nash Q-learning for finding an approximate Nash equilibrium, because the values of upper confidence and lower confidence---$\up{Q}$ and $\low{Q}$ will be eventually very close, so that the preconditions of Proposition \ref{prop:CCE} becomes approximately satisfied.


% \chijin{discussion on CCE being collaborative}



% \subsection{Nash V-learning}


